Asymmetric Mempool DoS Security: Formal Definitions and Provable Secure Designs

The mempool plays a crucial role in blockchain systems as a buffer zone for pending transactions before they are executed and included in a block. However, existing works primarily focus on mitigating defenses against already identified real-world attacks. This paper introduces secure blockchain-mempool designs capable of defending against any form of asymmetric eviction DoS attacks. We establish formal security definitions for mempools under the eviction-based attack vector. Our proposed secure transaction admission algorithm, named \textsc{saferAd-CP}, ensures eviction-security by providing a provable lower bound on the cost of executing eviction DoS attacks. Through evaluation with real transaction trace replays, \textsc{saferAd-CP} demonstrates negligible latency and significantly high lower bounds against any eviction attack, highlighting its effectiveness and robustness in securing blockchain mempools.

==> sty/ieeetran/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/titlepage.tex <==
\input{sty/title.tex}
\author{
\ifdefined\TTUT
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\fi
}

\maketitle
\IEEEpeerreviewmaketitle



==> text/1_intro.tex <==



==> text/change_wanning.tex <==
\section{Implementation Notes on Geth}

We build a prototype implementation of \text{saferAd} on Geth $v1.11.4$. We describe how the pending mempool in vanilla Geth handles transaction admission and then how we integrate \textsc{saferAd} into Geth.

\noindent{\bf
Background: Geth mempool impl.}: In the mempool of Geth $v1.11.4$, each transaction is stored twice in two different data structures: a primary storage where transactions are ordered by price and a secondary index where transactions are ordered first by senders and then by nonces. 

Upon an arriving transaction $tx_i$, Geth first checks if the mempool is full. \circled{1} If so, it finds the transaction of the lowest fees as the candidate of eviction victim $te_i'$. \circled{2} It then removes $te_i'$ from the primary storage and the secondary index. \circled{3} At last, it adds $tx_i$ to the primary storage and the secondary index.

If the mempool is not full, \circled{4} Geth adds $tx_i$ to the primary storage and to the secondary index.

\noindent{\bf
Implementation of \textsc{saferAd} on Geth}: 
Algorithm~\ref{alg:saferadE} is aligned well with Geth's mempool implementation and can be naturally realized on Geth:
We hook the pre-checks in Line~\ref{alg:saferadE:2} in Algorithm~\ref{alg:saferadE} right before \circled{2} in Geth. 
%We hook Line~\ref{alg:saferadE:3} in Algorithm~\ref{alg:saferadE} right before \circled{4} in Geth. 

Geth $v1.11.4$ has been patched to mitigate DETER (i.e., checking future transactions and latent overdrafts). In addition, we implement additional rules to mitigate MemPurge attacks~\cite{me:mempurge:fix}.

Upon \circled{1}, given the candidate $te_i'$ found by Geth, we further find its descendant transaction $te_i$ by going through the secondary index. We use $te_i$ as the eviction-victim candidate instead of $te_i'$. 
%both \texttt{ckEvict} and \texttt{ckAdmit} (Line~\ref{alg:saferadE:1} and Line~\ref{alg:saferadE:2} in Algorithm~\ref{alg:saferadE}) are trivial if $map$ is given. 
For calculating $map$, we add an index that, for each sender account, maintains the lowest fees of all transactions associated with the sender. Our index is synchronously updated with the secondary index in Geth, that is, when the list of transactions from a sender (in the secondary index) is changed.

\section{Revenue Evaluation}

\subsection{Experimental Setups}
\label{sec:setup}

{\it Workload collection}: 
For transaction collection, we first instrumented a Geth client (denoted by Geth-m) to log every message it receives from every neighbor. The logged messages contain transactions, transaction hashes (announcements), and blocks. When the client receives the same message from multiple neighbors, it logs it as multiple message-neighbor pairs. We also log the arrival time of a transaction or a block.


We ran a Geth-m node in the mainnet and collected transactions propagated to it from Sep. 5, 2023 to Oct. 5, 2023. In total, $1.5*20^8$ raw transactions are collected, consuming $30$ GB-storage. 
We make the collected transactions replayable as follows: We initialize the local state, that is, account balances and nonces by crawling relevant data from infura.io. We then replace the original sender in the collected transactions with the public keys that we generated. By this means, we know the secret keys of transaction senders and are able to send the otherwise same transactions for experiments. 

We choose $8$ traces of consecutive transactions from the raw dataset collected, each lasting $2.5$ hour. We run experiments on each $2.5$-hour trace. The reason to do so, instead of running experiments directly on the one-month transaction trace, is that the initialization of blockchain state in each trace requires issuing RPC queries (e.g., against infura) on relevant accounts, which is consuming; for a $2.5$-hour trace, the average time of RPC querying is about one day. To make the selected $2.5$-hour traces representative, we cover both weekdays and weekends, and on a single day, daytime and evening times.


\begin{figure}[!bthp]
\centering
%\includegraphics[width=0.375\textwidth]{figures/exp-setup.eps}
\includegraphics[width=0.375\textwidth]{figures/exp-setup2.eps}
\caption{Experimental setup}
\label{fig:exp:setup}
\end{figure}

{\it Experimental setup}:
For experiments, we set up four nodes, an optional attack node sending crafted transactions, a workload node sending normal transactions collected, a victim non-validator node propagating the transactions and blocks between attack node and victim validator node, and a victim validator node receiving transactions from the workload node and attack node through non-validator node. The victim validator node is connected to both the workload node and victim non-validator node which is connected to the attack node. There is no direct connection between the attack node and the workload node. The attack node runs an instrumented Geth $v1.11.4$ client (denoted by Geth-a) that can propagate invalid transactions to its neighbors. The victim nodes runs the target Ethereum client to be tested; we tested two victim clients: vanilla Geth $v1.11.4$ and \textsc{saferAd} $map$; the latter one is implemented as addon to Geth $v1.11.4$. The workload node runs a vanilla Geth $v1.11.4$ client. On each node, we also run a Prysm $v3.3.0$ client at the consensus layer. The experiment platform is depicted in Figure~\ref{fig:exp:setup}.
Among the four nodes, we stake Ether to the consensus-layer client on the victim validator node, so that only the victim validator node would propose or produce blocks. 

We run experiments in two settings: under attacks and without attacks. For the former, we aim at evaluating the security of \textsc{saferAd} under attacks, that is, how successful DoS attacks are on \textsc{saferAd}. In this setting, we run all three nodes (the victim, attacker and workload nodes). For the latter, we aim at evaluating the utility of \textsc{saferAd} under normal transaction workloads. In this setting, we only run victim and workload nodes, without running the attacker node.

In each experiment, 1) we replay the collected transactions as follows: For each original transaction $tx$ collected, we send a replayed transaction $tx'$ by replacing its sender with a self-generated blockchain address. $GasUsed$ is simulated: If $tx$ runs a smart contract, $tx'$ does not run the same contract. Instead, we make $tx'$ run our smart contract with $tx'.GasUsed$ equals $tx.GasUsed$ if $tx$ is included in the mainnet blockchain, or equal $tx.Gas$ (i.e., the Gas limit set by the transaction sender) if $tx$ is not included.
2) When replaying a collected block, we turn on the block-validation function in Prysm, let it produce and validate one block, and send the block (which should be different from the content of the collected block) to the Geth client. We then immediately turn off block validation before replaying the next transaction in the trace.


\subsection{Revenue Under Normal Transactions}

This experiment compares different mempool policies by evaluating their block revenue under the same transaction workloads. 

We consider two mempool policies, the baseline one in Geth $v1.11.4$ and \textsc{saferAd}-$map$ on the baseline. Given each policy, we replay the $8$ transaction traces in the same way as before and collect the blocks produced. We report the total revenue (i.e., the total transaction fees) collected from the blocks and the average revenue per block. The results are presented in Figure~\ref{fig:Revenue_block_real_trace} and Table~\ref{tab:revenue:8traces}. Figure~\ref{fig:Revenue_block_real_trace} illustrates the revenue of $150$ blocks (i.e., $1/4$ of the blocks under Trace $2$) over time. The revenue of the three mempool policies are very close and fluctuate in a similar fashion. Table~\ref{tab:revenue:8traces} presents aggregated results in total revenue and revenue per block. Compared to the baseline of vanilla Geth $v1.11.4$, \textsc{saferAd}-$map$ has an average revenue per block falling in Range $[100\%-1.33\%, 100\%+2.55\%]$. This result shows that \textsc{saferAd} policy doesn't significantly change block revenue under the workload of normal transactions.


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.38\textwidth]{figures/Revenue_block_real_trace_ndss.eps}
  \caption{Block revenue w/w.o. \textsc{saferAd} under Trace $2$.}
\label{fig:Revenue_block_real_trace}
\end{figure}


\begin{table}[!htbp]
\caption{Block revenue of 8 real transaction traces under different policies. Bold are max and min numbers.}
\label{tab:revenue:8traces}
\centering{\small
\begin{tabularx}{0.495\textwidth}{|c|C|X|c|c| }
\hline 
Tx   & \multicolumn{2}{l|}{Policy $map$ (Ether)} & \multicolumn{2}{l|}{Geth (Ether)}  \\ \cline{2-5}
trace & Total revenue & Revenue per block & Total &Per block \\ \hline
1 & 
$429.38$	&$0.72 (+1.02\%)$
&$425.04$	&$0.71$	 \\ \hline
2&
$647.25$	&$1.08 (-1.19\%)$
&$655.05$	&$1.09$	\\ \hline
3 &
$487.55$	&$0.81 (-0.21\%)$	
&$488.57$	&$0.81$	 \\ \hline
4 &
$322.66$	&\textbf{0.54 (+2.55\%)}	
&$314.63$	&$0.52$	 \\ \hline   
5 &
$430.31$	&$0.72 (-1.09\%)$	
&$435.05$	&$0.73$	 \\ \hline
6 &
$674.48$	&\textbf{1.12 (-1.33\%)}	
&$683.57$	&$1.14$	 \\ \hline
7  & 
$339.68$	&$0.57 (+2.1\%)$	
&$332.69$	&$0.55$	 \\ \hline
8 &
$355.25$	&$0.59 (+0.74\%)$	
&$352.64$	&$0.59$	 \\ \hline
\end{tabularx}
}
\end{table}


\subsection{Revenue Under Attacks}
\label{sec:setup:singlenode}

This experiment evaluates the security of \textsc{saferAd} against known attacks. Given that our implementation is on Geth $v1.11.4$, we choose the attacks still effective on this version: $XT_6$~\cite{wang2023understanding}. Briefly, the attack works in four steps: 1) It first evicts the Geth mempool by sending $384$ transaction sequences, each of $16$ transactions from a distinct sender. The transaction fees are high enough to evict normal transactions initially in the mempool. 2) It then sends $69$ transactions to evict $69$ parent transactions sent in step 1) and turn their child transactions into future transactions. 3) Since now there are more than $5120$ pending transactions in the mempool, Geth's limit of $16$ transactions per send is off. It then conducts another eviction; this time, it sends all $5120$ transactions from one sender, evicting the ones sent in the previous round. 4) At last, it sends a single transaction to turn all transactions in the mempool but one into future transactions. The overall attack cost is low, costing the fee of one transaction.

Because $XT_6$ can evict Geth's mempool to be left with one transaction, we use as Geth's bound the maximal price in a given mempool times the maximal Gas per transaction (i.e., block Gas limit, namely $30$ million Gas).

We set up the experiment platform described in \S~\ref{sec:setup:singlenode}. In each experiment, we drive benign transactions from the workload node. Note that the collected workload contains the timings of both benign transactions and produced blocks. On the $30$-th block, we start the attack. The attacker node observes the arrival of a produced block and waits for $d$ seconds before sending a round of crafted transactions. 

The attack phase lasts for $36$ blocks; after the $66$-th block, we stop the attack node from sending crafted transactions. We keep running workload and victim nodes for another $24$ blocks and stop the entire process at the $90$-th block. We collect the blocks produced and, given a block, we report the total fee of transactions included. 

\begin{figure}[!ht]
  \centering
  \subfloat[$XT_6$ w. $8$-sec. delay (single node)]{%
\includegraphics[width=0.225\textwidth]{figures/saferad-attack-evaluation.eps}
    \label{fig:saferad-attack-eval}
    \label{fig:successrate-geth}}%
  \subfloat[$XT_6$ w. varying delay (single node)] {%
   \includegraphics[width=0.225\textwidth]{figures/saferad-attack-varying-delay.eps}
  \label{fig:delay-geth}}
  \caption{Validator revenue under attacks: With and without \textsc{saferAd} defenses.}%
\end{figure}

Figure~\ref{fig:saferad-attack-eval} reports the metrics for $XT_6$ on two victim clients: vanilla Geth $v1.11.4$ and \textsc{saferAd} $map$. Before the attack is launched (i.e., before the $30$-th block), the two clients produce a similar amount of fees for benign transactions, that is, around $0.7 - 2.0$ Ether per block. As soon as the attack starts from the $30$-th block, Geth's transaction fees quickly drop to zero Ether, which shows the success of $XT_6$ on unpatched Geth $v1.11.4$. There are some sporadic spikes (under $0.7$ Ether per block), which is due to that $XT_6$ cannot lock the mempool on Geth. 
Patching Geth with \textsc{saferAd}-$map$ can fix the vulnerability. After the attack starts on the $30$-th block, the transaction fees, instead of decreasing, actually increase to a large value; the high fees are from adversarial transactions and are charged to the attacker's accounts. The high fees show the effectiveness of \textsc{saferAd} against known eviction-based attacks ($XT_6$).



Figure~\ref{fig:delay-geth} shows the total fee per block under $XT_6$ with varying delays, where the delay measures the time between when a block is produced and when the next attack arrives.
The results of Geth $v1.11.4$ show that with a short delay, the total transaction fees in mempool are high because $XT_6$ cannot lock a mempool, and the short block-to-attack delay leaves enough time to refill the mempool. With a median delay (e.g., sending an attack $8$ seconds after a block is produced), the attack is most successful, leaving mempool at zero Ether. With a long delay, the in-mempool transaction fees grow high due to the attack itself being interrupted by the block production. Under varying delays, the transaction fees of the mempool practicing \textsc{saferAd}-$map$ policy would remain constant at a high value, showing the defense effectiveness against attacks of varying delays.


\subsection{Estimation of Eviction Bounds}
\label{sec:eval:eviction:bounds}

{\color{blue}

}

This experiment evaluates the eviction bound of \textsc{saferAd}, as in Equation~\ref{eqn:mf:bound}, under real-world transaction workloads. 

Our goal is to understand whether bounding mempool fees using Equation~\ref{eqn:mf:bound} ensures the failure of known ADAMS attacks. In that regard, we also include a baseline, namely, the fees of an unprotected mempool under a successful ADAMS attack.

\ignore{
This experiment quantitatively evaluates the different eviction fee bounds for \textsc{saferAd}-$map$ and unprotected Geth $v1.11.4$. Recall that the lower bound of transaction fees for \textsc{saferAd}-$map$ is dependent on the benign transaction workloads (e.g., $st_{nb}$ as in Equation~\ref{eqn:mf:bound}). We evaluate the bound in the equation on real-world transaction traces collected from the mainnet.
}

% comparing with the total fees in the mempool without attack
% For vanilla Geth $v1.11.4$, as mentioned in Section $5.3$, the mempool fees under $XT_6$ attack correspond to the fee of the highest-priced transaction that remains.



In this experiment, we replayed eight real-world transaction traces to test two Ethereum clients: vanilla Geth $v1.11.4$ and Geth hardened with \textsc{saferAd}-$map$. We replayed the traces on vanilla Geth $v1.11.4$ twice and on \textsc{saferAd}-$map$ once. On each run, we captured snapshots every 30 seconds and evaluated the following metrics: 
1) \textsc{saferAd} fee bound: the eviction bound estimate using Equation~\ref{eqn:mf:bound}. 
2) Geth fees without attacks: that is  the total transaction fees in vanilla Geth $v1.11.4$ client without any attack. 
3) Geth fees with $XT_6$ attacks: that is the transaction fees in Geth $v1.11.4$ under $XT_6$ attack, where the mempool is evicted to a single transaction with the highest price.

% In the experiment, we test given clients: a vanilla Geth $v1.11.4$ and Geth hardened by \textsc{saferAd}-$map$. Given a tested client, we replay the collected eight transaction traces described in \S~\ref{sec:setup}. We take a snapshot every $30$ seconds, and estimate the lower bounds using the derived equation (Equation~\ref{eqn:mf:bound}). At each time point, given a mempool state $st$, we record three metrics: Total mempool fees in vanilla Geth $v1.11.4$ without attack, the eviction bound estimated from the \textsc{saferAd} mempool, and the mempool fees of vanilla Geth $v1.11.4$ under the $XT_6$ attack (the baseline). For the baseline, since $XT_6$ can evict the mempool to a single transaction, we conservatively use the transaction of the highest price in a mempool to estimate the fees.


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.38\textwidth]{figures/Block_revenue_lower_bound_ndss.eps}
  \caption{Block revenue lower bounds.}
\label{fig:Block_revenue_lower_bound_ndss}
\end{figure}

Figure~\ref{fig:Block_revenue_lower_bound_ndss} reports the timeline results of one trace (i.e., with mainnet transactions from 3:00 PM to 5:30 PM (UTC) on 09/05/2023) across different clients. The figure illustrates that \textsc{saferAd} tightly bounds the Geth fees without attack, with \textsc{saferAd}'s bounds being significantly higher compared to the original vanilla Geth client with $XT_6$ attack (baseline), by up to 4 orders of magnitude.

Table~\ref{tab:eviction:bound} presents the percentage ratios of estimated fee bounds under attacks to Geth fees without attack across eight transaction traces.
Our observations indicate that the bounds provided by \textsc{saferAd} are consistently high across all trace time periods. On average, the bound represents 34.18\% of Geth fees without attack, and notably, 5\% of lower bounds exceed 71\% of Geth fees.

% Table~\ref{tab:eviction:bound} presents the percentage of ratio for estimated fee bound under eviction attacks to mempool fees without attack across eight traces.
% Based on our observations, the bounds provided by \textsc{saferAd} are notably high. Specifically, we found that only 5\% of the snapshots have a lower bound that is less than 7.3\% of mempool fees without attack. Additionally, the average bound reaches $34.18\%$  of mempool fees, and remarkably, $5\%$ of lower bounds are higher than $71\%$ of mempool fees.

\begin{table}[!htbp]
\caption{Percentage ratios of \textsc{saferAd} fee bound (with attack) to $Geth$ fees (w.o. attack) across eight transaction traces}
\label{tab:eviction:bound}
\centering{\small
\begin{tabularx}{0.4\textwidth}{|l|X|X|X|}
\hline 
  & Avg. & $95\%$ & $5\%$\\ \hline
 \textsc{saferAd} & $34.18\%$	&$71.26\%$	&$7.3\%$ \\ \hline
 Geth & $2.2\cdot{}10^{-5}$	& $4.2\cdot{}10^{-5}$ &$8\cdot{}10^{-6}$ \\ \hline
\end{tabularx}
}
\end{table}

\subsection{Estimation of Locking Bounds}
\label{sec:eval:locking:bounds}

This experiment estimates the locking bounds of the declined transactions under \textsc{saferAd}. 
Recall that the locking security of \textsc{saferAd} is dependent on an assumption of benign transaction workloads, as stated in Equation~\ref{eqn:locking:assumption}. We evaluate the $\gamma$ value in this equation on real-world transaction traces collected from the mainnet.

Specifically, we collected transactions arriving at a node that we launched to join the Ethereum mainnet. We denote the transaction list by $\vec{ts_1}$. For each pending transaction $tx\in{}vec{ts_1}$, we obtain $\gamma(tx) = \frac{tx.price}{map(tx, \vec{ts_1})} - 1$. $\gamma$ is then as follows:

\begin{eqnarray}
\label{eqn:eval:gamma:sender}
\gamma(s) &=& \max_{\forall{}tx\in{}\vec{ts_1}\land{}tx.sender=s}\frac{tx.price}{map(tx, \vec{ts_1})} - 1
\\ 
\label{eqn:eval:gamma}
\gamma &=& \max_{\forall{}tx\in{}\vec{ts_1}}\frac{tx.price}{map(tx, \vec{ts_1})} - 1
\end{eqnarray}

\begin{table}[!htbp]
\caption{Estimated value of $\gamma$ from eight real transaction traces. $\gamma(>95\%)$ means $\gamma$ is higher than those of $95\%$ senders.}
\label{tab:locking:bound}
\centering{\small
\begin{tabularx}{0.46\textwidth}{|c|c|c|c|X| }
\hline 
 Tx trace & $\gamma$ (avg) & $\gamma$ (max) & $\gamma$ ($>95\%$) & $\gamma$ ($>50\%$)\\ \hline
 1 &
$0.8253$	&$19.0$	&$6.58$	&$0.0$
 \\\hline
 2 &
 $0.3713$	&$8.11$	&$2.0$	&$0.01$
 \\\hline
  3 &
$0.336$	&$9.05$	&$2.4$	&$0.0$
 \\\hline
  4 &
$0.8498$	&\textbf{23.29}	&$6.91$	&$0.0$
 \\\hline
  5 &
$0.5072$	&$15.07$	&$4.0$	&$0.0$
 \\\hline
  6 &
$0.3769$	&$9.63$	&$2.63$	&$0.0$
 \\\hline
  7 &
\textbf{0.9247}	&$21.21$	&\textbf{7.404}	&$0.0$
 \\\hline
  8 &
$0.3502$	&$9.15$	&$2.513$	&$0.0$
\\ \hline
\end{tabularx}
}
\end{table}

In experiments, we use the eight transaction traces as described in \S~\ref{sec:setup}. The results are illustrated in Table~\ref{tab:locking:bound}. The maximal $\gamma$ (in Equation~\ref{eqn:eval:gamma}) are between $8.11$ and $23.29$ across the eight traces. We also report the distribution of $\gamma$ under a given sender $s$ (i.e., $\gamma(s)$ in Equation~\ref{eqn:eval:gamma:sender}), including the average $\gamma(s)$ across senders and the $\gamma(s)$ bound higher than $95\%$ senders. The maximal average $\gamma(s)$ is $0.9247$, and the $\gamma(s)$ upper bound above $95\%$ senders is $7.4$. This implies that under arbitrary attacks, the maximal price of declined transactions by a mempool running Algorithm~\ref{alg:saferadE} can be bounded by $23.29\times$ of the minimal price of transactions in the mempool. 

\section{Performance Evaluation}
\subsection{Platform Setup}

In this work, we use Ethereum Foundation's test framework~\cite{me:txpooltest} to evaluate the performance of the implemented countermeasures on Ethereum clients. Briefly, the framework runs two phases: In the initialization phase, it sets up a tested Ethereum client and populates its mempool with certain transactions. In the workload phase, it runs multiple ``rounds'', each of which drives a number of transactions generated under a target workload to the client and collects a number of performance metrics (e.g., latency, memory utilization, etc.). In the end, it reports the average performance by the number of rounds.
In terms of workloads, we use one provided workload (i.e., ``Batch insert'') and implement our own workload (``Mitigated attacks'').


\subsection{Experimental Results}

\noindent{\bf Workload ``Batch insert''}: 
We use the provided workload "Batch insert" that issues \texttt{addRemote} calls to the tested \texttt{txpool} of the Geth client. We select this workload because all our countermeasures are implemented inside the \texttt{addRemote} function. In the initialization phase, this workload sends no transaction to the empty mempool. In the workload phase, it runs one round and sends $n_0$ transactions from one sender account, with nonces ranging from $1$ to $n_0$, and of fixed Gas price $10000$ wei. When $n_0$ is larger than the mempool size, Geth admits the extra transactions to the mempool, buffers them, and eventually deletes them by running an asynchronous process that reorg the mempool (i.e., Function \texttt{pool.scheduleReorgLoop()} in Geth).

\begin{figure}[!ht]
\centering
\subfloat[Workload ``Batch insert'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_BatchInsert_ndss.eps}
   % \includegraphics[width=0.45\textwidth]{figures/wanning.eps}
    \label{fig:mentor-case}}
\subfloat[Workload ``Mitigated attack TN1'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_TD1_ndss.eps}
    \label{fig:corner-td1}}%
\caption{Running time of \textsc{saferAd} on Geth $v1.11.4$}%
\end{figure}

\begin{figure}[!ht]
\centering
\subfloat[Workload ``Batch insert'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_BatchInsert_memory_ndss.eps}
   % \includegraphics[width=0.45\textwidth]{figures/wanning.eps}
    \label{fig:mentor-case_memory}}
\subfloat[Workload ``Mitigated attack TN1'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_TD1_memory_ndss.eps}
    \label{fig:corner-td1_memory}}%
\caption{Memory usage of \textsc{saferAd} on Geth $v1.11.4$}%
\end{figure}

{
%\color{red}
We report running time and memory usage in Figure~\ref{fig:mentor-case} and Figure~\ref{fig:mentor-case_memory}, respectively. In each figure, we vary the number of transactions $n_0$ from $1000$ to $10000$, where $n_0 \in [1000, 5000]$ indicates a non-full mempool, and $n_0 \in [5000, 10000]$ indicates a full mempool. It is clear that on both figures, the performance overhead for a non-full mempool is much lower than that for a full mempool; and when the mempool is full, both the running time and memory usage linearly increase with $n_0$. The high overhead is due to the expensive mempool-reorg process triggered by a full mempool.
Specifically, 1) upon a full mempool ($n_0\leq{}5000$), on average, Geth $v1.11.4$ hardened by \textsc{saferAd} $map$ causes $1.073\times$ running time and $1.000\times$ memory usage, compared to vanilla Geth $V1.11.4$.
2) When the mempool is not full ($n_0\leq{}5000$), on average, Geth $v1.11.4$ hardened by \textsc{saferAd} $map$ causes $1.017\times$ running time and $1.000\times$ memory usage, compared to vanilla Geth $V1.11.4$.
Overall, the performance overhead introduced by \textsc{saferAd}-$map$ is negligible.
} 

Note that Geth $v1.11.4$ that mitigates DETER causes $1.083\times$ running time compared to vanilla Geth $v1.11.3$, which is vulnerable to DETER. 


\noindent{\bf Workload ``Mitigated attack TN1''}: 
We additionally extend the framework with our custom workloads for countermeasure evaluation. Here, we describe the performance under one custom workload, "Mitigated attack TN1".

In the initialization phase, it first sends $n_1$ pending transactions to an empty mempool sent from $n_1'$ accounts, each of which has transactions of nonces ranging from $1$ to $\frac{n_1}{n_1'}$. All the parent transactions of nonce $1$ are of Gas price $1,000$ wei, and the others are of $200,000$ wei. It then sends $1024$ future transactions and $5120-n_1$ pending transactions from different accounts, all with nonce $1$, to fill the mempool. In the workload phase, it sends $n_1'$ transactions, each of price $20,000$ wei, to evict the parents and turn children into future transactions. 

In each experiment, we fix $n_1'$ at $10$ accounts and vary $n_1$ to be $10, 100, 1000$ and $4000$. We run the workload ten times and report the average running time and memory used with the standard deviation, as in Figure~\ref{fig:corner-td1} and Figure~\ref{fig:corner-td1_memory}. The running time and memory used are insensitive to the number of transactions ($n_1$). The performance overhead introduced by \textsc{saferAd} policy $map$ is negligible.

\section{Conclusion}

This paper presents provenly secure mempool designs under asymmetric DoS attacks. It formulates security definitions under two abstract DoSes, namely eviction- and locking-based attacks. It presents a suite of secure mempool policies, \textsc{saferAd}, that achieves both eviction- and locking- security. The evaluation shows \textsc{saferAd} incurs negligible overhead in latency and validator revenue.

==> text/paper101.tex <==
\section{Introduction}

In public blockchains, a mempool is a data structure residing on every blockchain node, responsible for buffering unconfirmed transactions before they are included in blocks. On Ethereum, mempools are present in various execution-layer clients serving public transactions, such as Geth~\cite{me:geth}, Nethermind~\cite{me:nethermind}, Erigon~\cite{me:erigon}, Besu~\cite{me:besu}, and Reth~\cite{me:reth}. They are also utilized by block builders managing private transactions within the proposer-builder separation architecture, such as Flashbots~\cite{me:flashbotbuilder}, Eigenphi~\cite{me:eigenphibuilder}, and BloXroute builders~\cite{me:bloXroutebuilder}.

Unlike conventional network stacks, mempools are permissionless and must accept transactions from unauthenticated accounts to maintain decentralization. This open nature, while essential for decentralization, makes the mempool vulnerable to denial-of-service (DoS) attacks. In such an attack, an adversary infiltrates the target blockchain network, establishes connections with victim nodes, and floods them with crafted transactions to deny mempool services to legitimate transactions. The disruption of mempool services can severely impact various blockchain subsystems, including block building, transaction propagation, blockchain value extraction (e.g., MEV searching), remote-procedure calls, and Gas stations. For instance, empirical studies have shown that disabling mempools can force the Ethereum network to produce empty blocks, undermining validators' incentives and increasing the risk of 51\% attacks.

\noindent{\bf Related works \& open problems}:
Denial of mempool services have been recently recognized and studied in both the research community and industry. In a large-scale blockchain, a mempool of limited capacity has to order transactions by certain priority criteria for transaction admission and eviction. The admission policy can be exploited to mount mempool DoS. The early attack designs~\cite{DBLP:conf/fc/BaqerHMW16,DBLP:conf/icbc2/SaadNKKNM19} work by sending spam transactions of high prices to evict benign transactions of normal prices. These attacks are extremely expensive and are not practical. 

Of more realistic threat is the {\it Asymmetric} DeniAl of Mempool Service, coined by us as ADAMS attacks, where the attacker spends much less fees in the adversarial transactions he sends than the damage he caused, that is, the fees of evicted benign transactions that would be otherwise chargeable. DETER~\cite{DBLP:conf/ccs/LiWT21} is the first ADAMS attack studied in research works where the attacker sends invalid and thus unchargeable transactions (e.g., future transactions in Ethereum) to evict valid benign transactions from the mempool. 
The MemPurge attack~\cite{cryptoeprint:2023/956} similarly evict Ethereum's (more specifically, Geth’s) pending-transaction mempool by crafting invalid overdraft transactions. 
These ADAMS attacks follow a single-step pattern and can be easily detected. In fact, DETER bugs have been fixed in Geth $v1.11.4$~\cite{me:gethfix11:thirdparty}, and there is a code fix implemented and tested against MemPurge on Geth~\cite{me:gethfix11:mempurge}. 

More sophisticated and stealthy attacks are recently discovered by \textsc{mpfuzz}, a symbolized stateful fuzzer for testing mempools~\cite{wang2023understanding}. The discovered attacks transition mempool states in multiple steps (see \S~\ref{sec:setup:singlenode} for an example exploit, $XT_6$) and are stealthy to detection. They can evade the mitigation designed for earlier and simpler ADAMS attacks. For instance, Geth $v1.11.4$, which is already patched against DETER attacks, is found still vulnerable by \textsc{mpfuzz}, such as under the $XT_6$ attack~\cite{wang2023understanding}.


Current defenses against mempool DoS attacks typically involve patching vulnerabilities after specific attack patterns have been identified. This reactive approach, while necessary, cannot fully guarantee eviction security for the mempool, as there may be undiscovered attacks capable of bypassing these patches. Therefore, the key to ensuring robust mempool security lies in a formal understanding of mempool DoS security. Without a precise security definition, it is impossible to validate or certify the soundness or completeness of a mempool's defenses against unknown attacks, let alone design new mempools with provable security. Notably, the bug oracles used in tools like \textsc{mpfuzz} optimize search efficiency but do not guarantee completeness, further highlighting the need for a comprehensive security framework.

Note that ADAMS attacks that exploit mempool admission policies are not the only means to cause under-utilized blocks in a victim blockchain. There are other DoS vectors, notably the computing-resource-exhaustion attacks targeting any blockchain subsystems prior to block validation. Known exhaustion strategies include running under-priced smart-contract instructions~\cite{DBLP:conf/ndss/0002L20,me:eip150,me:dosblockgas} or exploiting ``speculative’’ contract execution capabilities, such as the \texttt{eth\_call} in Ethereum’s RPC subsystem~\cite{DBLP:conf/ndss/LiCLT0L21} or censorship enforcement in Ethereum PBS (proposer-builder separation) subsystem (i.e., the ConditionalExhaust attack in~\cite{cryptoeprint:2023/956}). Resource exhaustion by adversarial smart contracts is out of the scope of this paper. Besides, denial of blockchain services have been studied across different layers in a blockchain system stack including eclipse attacks on the P2P networks~\cite{DBLP:conf/uss/HeilmanKZG15,DBLP:journals/iacr/MarcusHG18,DBLP:conf/sp/ApostolakiZV17,tran2020stealthier}, DoS blockchain consensus~\cite{mirkin2019bdos,me:finney}, DoS state storage~\cite{me:NURGLEDosstorage}, etc.

This work formulates the economic-security notions to protect mempools against asymmetric eviction DoS attacks. Economic security entails fee calculation, which may be non-deterministic in Ethereum and poses challenges in mempool designs. This work focuses on the mempool DoS by exploiting transaction admission policies, which normally rely only on deterministic transaction prices and are agnostic to non-deterministic Gas or fees. 

\noindent{\bf Proposed policy}: This work presents the first definitions of asymmetric eviction mempool DoS security and the provably secure mempool designs. Specifically, we conceive a general pattern of mempool eviction-based DoSes: Attackers aim to evict the victim transactions residential in a mempool. Based on the pattern, we formulate a security definition, that is, $g$-eviction security, which requires a secure mempool to lower bound the total fees of residential transactions under arbitrary sequences of transaction arrivals. 
%Note that all known mempool DoSes, including DETER and MemPurge, cause violation of eviction security without violating locking security.


This work presents \textsc{saferAd}-$PR$, a transaction admission policy for securing mempools against asymmetric eviction DoSes. \textsc{saferAd}-$PR$ can achieve eviction security by lower-bounding the fees of any arriving transactions causing eviction which is much higher than original Geth. We focus on designing admission policy in a pending-transaction mempool, that is, the pool is supposed to store only valid transactions (whereas future or other invalid transactions are buffered in a separate pool).\footnote{In the rest of the paper, the term mempool refers only to the pool storing pending transactions.} 

\textsc{saferAd}-$PR$ prevents valid residential transactions from being turned into invalid ones by evicting only ``child-less'' transactions, that is, the ones with the maximal nonce of its sender.
Upon each arriving transaction, if the transaction is admitted by evicting another transaction, it enforces that the fee of the admitted transaction must not be lower than a pre-set lower bound. 
%Under this framework, we propose two specific admission policies, named Policy $mf$ and E. 

\noindent{\bf Evaluation}:
We analyze \textsc{saferAd}-$PR$ and prove the eviction-based DoS security with eviction bound: lower-bound the attack costs (i.e., the adversarial transaction fees) under eviction DoSes.

We implement a \textsc{saferAd}-$PR$ prototype over Geth by evicting only ``child-less'' transactions. We collect real-world transactions from the Ethereum mainnet, and replay them against the \textsc{saferAd}-$PR$ prototype. The evaluation shows \textsc{saferAd}-$PR$ incurs a revenue change between $[+1.18\%, +7.96\%]$ under replayed real-world transaction histories. \textsc{saferAd}-$PR$'s latency in serving transactions is at most $7.3\%$ different from a vanilla Geth client. Under the attacks that latest Geth is known to be vulnerable for, \textsc{saferAd}-$PR$ increases the attacker's cost by more than $10^4$ times.

\noindent{\bf Contributions}:
Overall, this paper makes the following contributions:

\vspace{2pt}\noindent$\bullet$\textit{ 
New security definitions}:
Presented the first economic-security definitions of mempools against asymmetric eviction DoSes. Specifically, we formulate a general pattern of mempool eviction DoSes and present a security definition to mitigate this attack pattern.

\vspace{2pt}\noindent$\bullet$\textit{ 
Proven secure designs}:
Presented the first eviction DoS-secure mempool designs, \textsc{saferAd}-$PR$, that achieves proven eviction-based security. The security stems from \textsc{saferAd}-$PR$'s design in lower-bounding the attack cost under eviction DoSes.

\vspace{2pt}\noindent$\bullet$\textit{ 
Performance \& utility evaluation}:
Implemented a \textsc{saferAd}-$PR$ prototype on Geth and evaluated its performance and utility by replaying real-world transaction traces. It shows \textsc{saferAd}-$PR$ incurs negligible overhead in latency and maintains a high lower bound on validator revenue under any adversarial traces.

\section{Background and Notations}
\noindent{\bf Transactions}: In Ethereum, a transaction $tx$ is characterized by a $sender$, a $nonce$, a $price$, an amount of computation it consumes, $GasUsed$, and the $data$ field relevant to smart-contract invocation. Among these attributes, transaction $sender$, $nonce$, and $price$ are ``static'' in the sense that they are independent of smart contract execution or the context of block validation (e.g., how transactions are ordered). This work aims at lightweight mempool designs leveraging only static transaction attributes. We denote an Ethereum transaction by its $sender$, $nonce$, and $price$. For instance, a transaction $tx_1$ sent from Account $A$, with nonce $3$, of price $7$ is denoted by $\langle{}A3, 7\rangle{}$.

A transaction $tx_1$ is $tx_2$'s ancestor or parent if $tx_1.sender=tx_2.sender\land{}tx_1.nonce<tx_2.nonce$. We denote the set of ancestor transactions to transaction $tx$ by $tx.ancestors()$. Given the transaction set in a mempool state $ts$, $tx$'s ancestor transactions in $ts$ and with consecutive nonces to $tx$ are denoted by set $tx.ancestors()\cap{}ts$. For instance, suppose transactions $tx_1,tx_2,tx_3, tx_4$ are all sent from Alice and are with nonces $1$, $2$, $3$, and $4$, respectively. Then, $tx_4.ancestors()\cap{}\{tx_1, tx_3\text{\}}=\{tx_3\text{\}}$.

A transaction $tx$ is a future transaction w.r.t. a transaction set $ts$, if there is at least one transaction $tx'\not\in{}ts$ and $tx'$ is an ancestor of $tx$. Given any future transaction $tx$ in set $ts$, we define function $\textsc{isFuture}(tx, ts)=1$. 


\noindent{\bf Transaction fees}: A transaction $tx$'s fee is the product of $GasUsed$ and $price$, that is, $tx.fee=GasUsed\cdot{}price$. $GasUsed$ is determined by a fixed amount ($21000$ Gas) and the smart contract execution by $tx$. In Ethereum, The latter factor is sensitive to various runtime conditions, such as how transaction $tx$ is ordered in the blocks. After EIP-1559, part of price and fees are burnt; in this case, block revenue excludes the burnt part.


% \noindent{\bf Transactions}: In Ethereum, a transaction $tx$ is characterized by a $sender$, a $nonce$, a $price$, and an amount of computation it consumes, $GasUsed$. 

% A transaction $tx_1$ is another $tx_2$'s ancestor or parent, if $tx_1.sender=tx_2.sender\land{}tx_1.nonce<tx_2.nonce$ . We denote the set of ancestor transactions to transaction $tx$ by $tx.ancestors()$. Given a transaction set $ts$, $tx$'s ancestor transactions in $ts$ and with consecutive nonces to $tx$ are denoted by set $tx.ancestors(ts)$. For instance, suppose transactions $tx_1,tx_2,tx_3, tx_4$ are all sent from Alice and are with nonces $1$, $2$, $3$, and $4$, respectively. Then, $tx_4.ancestors(\{tx_1, tx_3\})=\{tx_3\}$ .

% A transaction $tx$ is a future transaction w.r.t. a transaction set $ts$, if there is at least one transaction $tx'\not\in{}ts$ and $tx'$ is an ancestor of $tx$. Given any future transaction $tx$ in set $ts$, we define function $\textsc{isFuture}(tx, ts)=1$. 

% A transaction $tx$'s fee is the product of $GasUsed$ and $price$, that is, $tx.fee=GasUsed\cdot{}price$. $GasUsed$ is determined by a fixed amount ($21000$ Gas) and the smart contract execution by $tx$. The latter factor in Ethereum is non-deterministic and is sensitive to various runtime factors, such as how transaction $tx$ is ordered in the blocks. 

% Before EIP-1559,  transaction fees are collected only by block validators as part of their revenue. After EIP-1559, fees or $price$ consist of two components: $price=BaseFee+PriorityFee$, where the $BaseFee$ is decided jointly by validators, and the associated fees are burnt upon transaction inclusion. The $PriorityFee$ or so-called $tip$ is collected by the validator. 

% A validator's revenue comes from two sources: transaction fees and bribes. Bribing refers to a transaction sender directly transferring assets, either Ether or tokens, to a validator so that the transaction can be favored for early block inclusion. Bribes can be specified in the $value$ field of an Ethereum transaction or in smart contracts.

% The notations used in this paper (some of which are introduced later in the paper) are listed in Table~\ref{tab:notations}. Notably, we differentiate the unordered set and ordered list: Given an unordered transaction set, say $ops$, an ordered list of the same set of transactions is denoted by a vector, $\vec{ops}$. A list is converted to a set $ops$ by the function $unorder(\vec{ops})$, and a set is converted to a list $\vec{ops}$ by the function $toOrder(ops)$.


\noindent{\bf The notations} used in this paper (some of which are introduced later in the paper) are listed in Table~\ref{tab:notations}. Notably, we differentiate the unordered set and ordered list: Given an unordered transaction set, say $ops$, an ordered list of the same set of transactions is denoted by a vector, $\vec{ops}$. A list is converted to a set $ops$ by the function $unorder(\vec{ops})$, and a set is converted to a list $\vec{ops}$ by the function $toOrder(ops)$.


\begin{table}[!htbp] %force in current page, disable float.
\caption{Notations: txs means transactions.}
\label{tab:notations}\centering{\footnotesize
\begin{tabularx}{0.49\textwidth}{ |l|X|l|X| }
  \hline
 & Meaning &  & Meaning  \\ \hline
$ops$ & Arriving txs
&
$\vec{ops}$ & List of arriving txs
\\ \hline
$st$ & Txs in mempool
&
$\vec{st}$ & List of txs in mempool
\\ \hline
$dc$ & Txs declined or evicted from mempool
&
$m$ & Mempool length 
\\ \hline
$\langle{}A3, 7\rangle{}$ 
& \multicolumn{3}{l|}{A tx of sender $A$, nonce $3$, and price $7$} 
\\ \hline
\end{tabularx}
}
\end{table}

\noindent{\bf Blockchain mempools}:
In blockchains, recently submitted transactions by users, a.k.a., unconfirmed transactions, are propagated, either privately or publicly, to reach one or multiple validator nodes. Mempool is a data structure a blockchain full node uses to buffer the ``unconfirmed'' transactions before these transactions are included in blocks. 

In Ethereum 2.0, transaction propagation follows two alternative paths. A public transaction is propagated to the entire network, while a private transaction is forwarded by a builder to the proposers who he has established the connection with. 
In both scenarios, the mempool faces the same design issues: Because the mempool needs to openly accept a potentially unlimited number of transactions sent from arbitrary EOA accounts, it needs to limit the capacity and enforce policies for transaction admission. In practice, we found the mempool storing public transactions has the same codebase as that storing private mempool.\footnote{For instance, the mempool in Flashbot builder~\cite{me:flashbotbuilder} used to store both private and public transactions is a fork (with no code change) of the mempool storing only public transactions in Geth.}

\section{Threat Model}
\label{sec:threat}

\begin{figure}
  \centering
%  \includegraphics[width=0.425\textwidth]{figures/saferad-downstream.eps}
  \includegraphics[width=0.425\textwidth]{figures/saferad-downstream2.eps}
  \caption{Threat model of a victim mempool: In blue are downstream operators that rely on reading or writing the mempool. In dark blue are the operators in the private transaction path. }
  \label{fig:downstream}
\end{figure} 

% \noindent{\bf Adversary's goals and capacities}: 
In the threat model, an adversary node is connected, either directly or indirectly, to a victim node on which a mempool serves various downstream operators reading or inserting transactions. Figure~\ref{fig:downstream} depicts some example mempool-dependent operators, including a transaction sender who wants to insert her transaction to the mempool, a full node that reads the mempool to decide whether a received transaction should be propagated, a validator or PBS builder that reads the mempool and selects transactions to be included in the next block, an MEV searcher that reads the mempool to find profitable opportunities, a Gas-station service that reads the mempool to estimate appropriate Gas price for sending transactions, etc. 

The adversary's goal is two-fold: 1) Deny the victim mempool's service to these critical downstream operators. This entails keeping all normal transactions out of the mempool so that the transaction read/write requests from operators would fail. 2) Keep the adversary's cost asymmetrically low. This entails keeping the transactions sent by the adversary away from being included in the blockchain. 

The adversary has the capacity to craft transactions and send them to reach the victim mempool. In the most basic model, the adversary is directly connected to the victim node. In practice, the adversary may launch a super-node connected to all nodes and aim at attacking all of them or selecting critical nodes to attack (as done in DETER~\cite{DBLP:conf/ccs/LiWT21}). Alternatively, the adversary may choose to launch a ``normal'' node connected to a few neighbors and propagate the crafted transactions via the node to reach all other nodes in the network.








\section{Security Definition}
\label{sec:secdef}

To start with, we characterize two mempool states at any time: the set of transactions residing in the mempool denoted by $st$, and the set of transactions declined or evicted from the mempool denoted by $dc$. We also characterize the list of confirmed transactions included in produced blocks by $\vec{bks}=\{\vec{b}\}$ and the list of transactions arriving by $\vec{ops}$.

A mempool commonly supports two procedures: transaction admission and block building. We specify the first one, which is relevant to this work. 

\begin{definition}[Tx admission]
\label{def:txadmit}
Given an arriving transaction $tx_i$ at a mempool of state $st_i$, an admission algorithm $\textsc{adTx}$ would transition the mempool into an end state $st_{i+1}$ by admitting or declining $tx_i$ or evicting transactions $te_i$. Formally,

\begin{equation}
\textsc{adTx}(st_i, tx_i) \rightarrow{} st_{i+1}, te_i
\end{equation}
\end{definition}

\begin{definition}[Tx admission timeline]
\label{def:timeline}
In a transaction admission timeline, a mempool under test is initialized at state $\langle{}st_0, dc_0=\emptyset\rangle{}$, receives a list of arriving transactions in $\vec{ops}$, and ends up with an end state $\langle{}st_n, dc_n\rangle{}$. Then, a validator continually builds blocks from transactions in the mempool $st_n$ until it is empty, leading to eventual state $\langle{}st_l=\emptyset, dc_l=dc_n\rangle{}$ and newly produced blocks $\vec{bks_l}$ with transactions in $st_n$. This transaction-admission timeline is denoted by $f(\langle{}st_0, \emptyset\rangle{},\vec{ops})\Rightarrow{}\langle{}st_n, dc_n\rangle{}$. 
\end{definition}

As in the above definition, this work considers the timeline in which block arrival or production does not interleave with the arrival of adversarial transactions. We leave it to the future work for interleaved block arrival and attacks. In the following, we define the mempool security against asymmetric attacks.

\begin{definition}[Mempool eviction security]
\label{def:security:evict}
Consider any mempool that initially stores normal transactions $st_0$, receives a list of benign and adversarial transactions $\vec{ops}$ and converts to the end state $st_n$. 

The mempool is secure against asymmetric eviction attacks, or {\bf $g$-eviction-secure}, if.f. the total transaction fees under any adversarial transactions are higher than $g(st_0)$ where $g(\cdot)$ is a price function that takes as input a mempool state and returns a price value. Formally,

\begin{eqnarray}
\nonumber 
&& \forall{} st_n, \vec{ops},  
\exists \text{function } g(\cdot)
\\
&& \text{ s.t., } \forall{st_0}, fees(st_n) \geq{} g(st_0)
\end{eqnarray}
\end{definition}

The $g$-eviction-security definition ensures that under arbitrary attacks, the total fees of transactions inside the mempool are lower bound by a value dependent only on normal transactions in initial state. 
This definition reflects the following intuition: If the normal transactions in initial state can provide enough block revenue for validators, the $g$-security of mempool ensures the mempool under any adversarial workloads (i.e., attacks) have enough fees or enough block revenue for validators.

% \begin{definition}[Mempool locking security]
% \label{def:security:locking}
% Consider under attacks in which the mempool of initial state storing only benign transactions $\langle{}st_0, \emptyset\rangle{}$ receives a transaction sequence $\vec{ops}$ interleaved of adversarial and benign transactions, transitions its state, and reaches the end state $\langle{}st_{n}, dc_n\rangle{}$, as shown Equation~\ref{eqn:def:attacktimeline2}. 

% The mempool is said to be secure against asymmetric locking attacks, or {\bf $h$-locking-secure}, if.f. the maximal price of transactions declined or evicted in the end state under attacks, i.e., $dc_n$, is lower than a certain price function $h()$ on the end-state mempool under attacks, i.e., $h(st_n)$. Formally,

% \begin{eqnarray}
% \nonumber 
% && \forall{} st_0, \vec{ops},  
% \\
% \label{eqn:def:attacktimeline2}
% && f(\langle{}st_0, \emptyset\rangle{}, \vec{ops})\Rightarrow{} \langle{}st_n, dc_n\rangle{}
% \\
% \nonumber 
% &&\exists \text{function } h(\cdot)
% \text{ s.t., } max(dc_n.price) < h(st_n)
% \end{eqnarray}
% \end{definition}

% The $h$-locking-security definition ensures that the maximal price of declined or evicted transactions from the mempool is upper bound by that of the transaction staying in the mempool.



\section{\textsc{saferAd} Framework}

\subsection{Tx-Admission Algorithm of $PR$}
\begin{algorithm}[h]
\caption{\textsc{saferAd}-$PR$(MempoolState $st$, Tx $ta$)}
\small \label{alg:adTx:AA:framework}
\begin{algorithmic}[1]
\If{$\textsc{preCkV}(ta, st)==0$} \Comment{Precheck tx validity} 
\label{alg:adTx:AA:0}
  \State \Return $te=ta$; \Comment{Decline invalid $ta$} 
\EndIf
\State $\vec{tes}$=\textsc{torder}($st.findChildless(), PR(\cdot)$); 
\label{alg:adTx:AA:1}
\State $te$=$\vec{tes}$.lastTx();
\label{alg:adTx:AA:2}
\If{$\|st\| == m$}
\If{$ta.price \leq te.price $} \label{alg:adTx:AA:3}
 \State \Return $te=ta$; \Comment{Decline $ta$} 
\label{alg:adTx:AA:4}
\Else
  \State $st$.admit($ta$).evict($te$); 
\label{alg:adTx:AA:5}
\EndIf
\Else
%\If{$score(te, st) < score(ta, st)$}\label{alg:adTx:AA:6}
% \State \Return $te=ta$; \Comment{Decline $ta$} \label{alg:adTx:AA:7}
%\Else
  \State $st$.admit($ta$); \label{alg:adTx:AA:8}
  \State $te=$NULL; \label{alg:adTx:AA:9}
\EndIf
\end{algorithmic}
\end{algorithm}

The proposed Algorithm~\ref{alg:adTx:AA:framework} enforces the invariant that each admitted transaction to a mempool evicts at most one transaction from the mempool. 

The algorithm initially maintains a mempool of state $st$ and receives an arriving transaction $ta$. The algorithm decides whether and how to admit $ta$ and produces as the output the end state of the mempool and the evicted transaction $te$ from the mempool. In case that $ta$ is declined by the mempool, $te=ta$.


Internally, the algorithm first pre-checks the validity of $ta$ on mempool $st$ (in Line~\ref{alg:adTx:AA:0}). If $ta$ is a future transaction or overdrafts its sender balance, the transaction is deemed invalid and is declined from entering the mempool. The algorithm only proceeds when $ta$ passes the validity precheck.

It then sorts all childless transactions in mempool ($st.findChildless()$) in descendant order based on tx's price ($PR(\cdot)$). As described next, function $\vec{tes}=\textsc{torder}(st)$ produces a order of transactions in the mempool, denoted by $\vec{tes}$.
It selects the last transaction on this ordered list, denoted by $te$. That is, $te$ has the lowest score on $\vec{tes}$. 

If the mempool is full and $ta.price \leq te.price$ (Line~\ref{alg:adTx:AA:3}), the algorithm declines the arriving transaction $ta$, that is, $te=ta$ (Line~\ref{alg:adTx:AA:4}). Otherwise, if the mempool is full and $ta.price > te.price$, the algorithm admits $ta$ and evicts $te$ (Line~\ref{alg:adTx:AA:5}).

If the mempool is not full, the algorithm always admits $ta$ to take the empty slot (Line~\ref{alg:adTx:AA:8}).

% \begin{algorithm}[h]
% \caption{\textsc{saferAd}-$PR$(Tx $tx$, State $st$)}
% \small \label{alg:saferadP}
% \begin{algorithmic}[1]
% \If{$\|st\| == m$}
% \If{\textsc{isFuture}($tx, st$)$=1 \lor$ \textsc{isOverdraft}($tx, st$)$=1$} \Comment{Check validity} 
% \label{alg:saferad:0}
%   \State \Return $te=tx$; \Comment{Decline invalid $tx$} 
%   % \label{alg:saferad:0}
% \Else
% \If{\textsc{hasFuture}($ st$)$=1 \lor$ \textsc{hasOverdraft}($ st$)$=1$}
% \State $tes = findFuture(st)$
% \label{alg:saferad:1}
% \State $tes = tes.append(findOverdraft(st))$
% \label{alg:saferad:2}
% \State $st$.Admit($tx$);
% \State \Return $te = tes.random()$; 
% \Comment{Evict $te$, $tx$ admitted}
% \Else \State $tes = findChildless(st)$;
% \label{alg:saferad:3}
% \State $te = min(sorted(tes, PR(tx, st)))$
% \label{alg:saferad:4}
% \If {$PR(te, st) < PR(tx, st\cup{tx})$}
% \label{alg:saferad:5}
% \State $st$.Admit($tx$);
% \label{alg:saferad:6}
% \State $st$.Evict($te$);
% \label{alg:saferad:7}
% \State \Return $te$; \Comment{Evict $te$, $tx$ admitted}
% \Else 
% \State \Return $te=tx$;
% \Comment{No eviction; $tx$ declined}
% \label{alg:saferad:8}
% \EndIf
% \EndIf
% \EndIf
% \Else \Comment{Empty slots}
% \State $st$.Admit($tx$); 
% \label{alg:saferad:9}
% \State \Return NULL; \Comment{No eviction; $tx$ admitted}
% \label{alg:saferad:10}
% \EndIf
% \end{algorithmic}
% \end{algorithm}

% To start with, \textsc{saferAd}-$PR$ hardens a pending-transaction mempool which is supposed to only admit valid transactions while it's full, meaning $\|st\| == m$ (where $m$ is the maximum size of the mempool). Invalid transactions (the future or latent overdraft transactions) are checked and declined by our mempool in full state which mitigates the simple known attacks (e.g DETER and MemPurge).

% Specifically, In algorithm~\ref{alg:saferadP}, given transaction $tx$ arriving at the mempool of state $st$, it first checks the validity of the transaction $tx$ as of $st$ in Line~\ref{alg:saferad:0}. 

% Only if $tx$ is a valid pending transaction w.r.t. $st$, $tx$ will pass the check in Line~\ref{alg:saferad:0}. 
% And then, 
% Line~\ref{alg:saferad:1} and Line~\ref{alg:saferad:2} find the candidate list of future transactions or overdraft transactions in the mempool state $st$. If there is any desirable candidate, randomly select one eviction transaction $te$ from the list and admit the arriving transaction $tx$.

% Line~\ref{alg:saferad:3} finds the candidate list of childless transactions ($tes$) based on the current state ($st$). Here, $tes$ refer to all transactions that do not have any child transactions present in the current pool state. Formally,
% \begin{equation}
% \label{eqn:candidate:list}
% tes =  \{ t \in st \mid t.child() = \emptyset \}
% \end{equation}

% After candidate transaction list generation, Line~\ref{alg:saferad:4} chooses the last transaction in ordered list ($\vec{tes}$) by their prices as the eviction transaction ($te$).
% In particular, for a sorted list containing multiple transactions with the same minimum price, we adopt a strategy of randomly selecting one transaction. This approach is justified for three reasons: 
% \begin{enumerate}
%     \item Regardless of the secondary metric used, the eviction bound remains unchanged.
%     \item The random selection introduces variability in choosing the eviction transaction, making it a moving target.
%     \item This method avoids the computational overhead associated with introducing new metrics.
% \end{enumerate}

% Line~\ref{alg:saferad:5} checks if the price of the arriving transaction $tx$ is higher than the minimum price among the childless transactions ($te.price$) currently in the system's transaction pool state $st$. If the condition is not met, Line~\ref{alg:saferad:8} declines the transaction $tx$.

% If the transaction $tx$ passes the price check, Line~\ref{alg:saferad:6} admits the transaction $tx$ to the mempool $st$ and Line~\ref{alg:saferad:7} evicts a transaction $te$ from the mempool $st$.

% If the mempool $st$ is not full, namely $\|st\| < m$: then Line~\ref{alg:saferad:9} admits the transaction $tx$ into the mempool $st$ regardless of its validity, without evicting any transaction.


\subsection{Eviction Secure of $PR$}
Policy \textsc{PR} achieves eviction security in the sense that it ensures the total prices monotonically increase. 

Suppose a mempool runs Algorithm~\ref{alg:adTx:AA:framework} and transitions from state $st_i$ to $st_{i+1}$. No transaction in $st_i$ can be turned into a future transaction in $st_{i+1}$.
Because the eviction candidates can only be the childless transactions (Recall Line~\ref{alg:adTx:AA:1} in Algorithm~\ref{alg:adTx:AA:framework}).
% \begin{lemma}[No tx turning of \textsc{saferAd}-$PR$]
% \label{lmm:cp1:noturn}
% Suppose a mempool runs Algorithm~\ref{alg:adTx:AA:framework} and transitions from state $st_i$ to $st_{i+1}$. No transaction in $st_i$ can be turned into a future transaction in $st_{i+1}$.
% \end{lemma}

% \begin{proof}
% We prove this lemma by contradiction. Assume $tx\in{}st_i$
% is turned into a future transaction in $st_{i+1}$.

% There must be an ancestor of $tx$, say $tx'$, that is evicted from $st_{i+1}$ by Algorithm~\ref{alg:adTx:AA:framework}. Due to Line~\ref{alg:adTx:AA:2}, $tx'$ must be ordered the last on $\vec{st_i}$. Because $tx'$ is a parent of $tx$, $score_{\textsc{CP}}(tx', st_i) = +\infty$. Suppose $tx$'s descendent, say $tx''$, that has no further child in $st_i$. $score_{\textsc{CP}}(tx'', st_i)\neq{}+\infty<score_{\textsc{CP}}(tx', st_i)$ . In other words, $tx'$ should be ordered before $tx''$. Contradiction.  
% \end{proof}


\begin{lemma}[Monotonic price-increasing]
\label{thm:pr:mono} 
If a mempool runs Algorithm~\ref{alg:adTx:AA:framework}, the sum of transaction prices in the mempool monotonically increases, or the mempool is considered to be monotonic price-increasing. Formally,

\begin{equation}
\label{eqn:iterative:n}
\sum_{tx\in{}st_n} tx.price \geq \sum_{tx\in{}st_0} tx.price
\end{equation}
\end{lemma}

\begin{proof}
Consider that a mempool running Algorithm~\ref{alg:adTx:AA:framework} receives an arriving transaction $ta_i$ and transitions from state $st_i$ to $st_{i+1}$. We aim to prove that,
\begin{equation}
\label{eqn:pr:iterative:i}
\sum_{tx\in{}st_{i+1}} tx.price \geq \sum_{tx\in{}st_i} tx.price
\end{equation}

Now we consider three cases for state transition: 
1) $ta_i$ is declined, 
2) $ta_i$ is admitted by taking an empty slot in $st_i$ (i.e., no transaction is evicted), and 
3) $ta_i$ is admitted by evicting $te_i$.

In Case 1), $st_i=st_{i+1}$. Thus,
\begin{eqnarray}
\nonumber
\sum_{tx\in{}st_i} tx.price
&=& \sum_{tx\in{}st_{i+1}} tx.price
\end{eqnarray}

In Case 2), $st_{i+1}=\{ta_i$\text{\}}$\cup{}st_i$. Thus,

\begin{eqnarray}
\nonumber
\sum_{tx\in{}st_{i+1}} tx.price &=&  
\sum_{tx\in{}st_i\cup{}\{ta_i\text{\}}} tx.price 
\\ \nonumber &=& 
\sum_{tx\in{}st_i} tx.price  + ta_i.price 
\\ \nonumber &\geq{}& 
\sum_{tx\in{}st_i} tx.price
\end{eqnarray}

In Case 3), we denote by $st$ the set of transactions in both $st_i$ and $st_{i+1}$. That is, $st=st_i\cap{}st_{i+1}$. In Case 3), we have $st_{i+1}\setminus{}\{ta_i$\text{\}}$=st_i\setminus{}\{te_i$\text{\}}$=st$. Applying Line~\ref{alg:adTx:AA:3} in Algorithm~\ref{alg:adTx:AA:framework}, we can derive the following:

\begin{eqnarray}
\nonumber
\sum_{tx\in{}st_{i+1}} tx.price &=& 
\sum_{tx\in{}st\cup{}\{ta_i\text{\}}} tx.price
\\ \nonumber &=& 
\sum_{tx\in{}st} tx.price + ta_i.price
\\ \nonumber &\geq{}& 
\sum_{tx\in{}st} tx.price + te_i.price 
\\ \nonumber &=& 
\sum_{tx\in{}st\cup{}\{te_i\text{\}}} tx.price 
\\ \nonumber &=& 
\sum_{tx\in{}st_i} tx.price
\end{eqnarray}

Therefore, in all three cases, Equation~\ref{eqn:pr:iterative:i} holds. In general, for any initial state $st_0$ and any end state $st_n$ that is transitioned from $st_0$ with $i\in[0,n-1]$, one can iteratively apply Equation~\ref{eqn:pr:iterative:i} for $i\in[0,n-1]$ and prove the sum of transaction price monotonically increases. 
\end{proof}


% \begin{proof}
% Suppose a mempool running Algorithm~\ref{alg:saferadP} transitions a state $st_i$ to $st_{i+1}$. We aim to prove that,
% \begin{equation}
% \label{eqn:iterative:i}
% \sum_{tx\in{}st_{i+1}} PR(tx, st_{i+1}) \geq \sum_{tx\in{}st_i} PR(tx, st_i)
% \end{equation}

% We consider three cases of transition: 1) by admitting transaction $tx$ and evicting $te$, 2) by admitting transaction $tx$ and evicting nothing, and 3) by declining transaction $tx$. We denote other transactions (not admitted or evicted) as $st_i''$. 

% For case 1), it is to prove,
% \begin{eqnarray}
% \label{eqn:proof:1}
% \sum_{tx'\in{}st_i''} PR(tx', st_{i+1}) + PR(tx, st_{i+1}) 
% \nonumber
% \\ 
% \geq \sum_{tx'\in{}st_i''} PR(tx', st_i) + PR(te, st_i)
% \end{eqnarray}

% Recall Line~\ref{alg:saferad:5} in Algorithm~\ref{alg:saferadP}, the transaction admission increase the $PR$ of the mempool slot admitting the transaction and admission or eviction of descendent transaction does not affect the $PR$ of transactions in $st_i''$. Formally,

% \begin{eqnarray}
% \label{eqn:saferAd:property:1}
% &&
% PR(tx, st_{i+1}) > PR(te, st_i) 
% \\ \nonumber
% &&
% \label{eqn:saferAd:property:2}
% \sum_{tx'\in{}st_i''} PR(tx', st_i) = \sum_{tx'\in{}st_i''} PR(tx', st_{i+1})
% \end{eqnarray}    
% Equation~\ref{eqn:proof:1} holds, and we conclude the proof for Case 1.


% For case 2), it is to prove,
% \begin{eqnarray}
% \label{eqn:proof:2}
% \sum_{tx'\in{}st_i''} PR(tx', st_{i+1}) + PR(tx, st_{i+1}) 
% \nonumber
% \\ 
% \geq \sum_{tx'\in{}st_i''} PR(tx', st_i) 
% \end{eqnarray}

% Because admission or eviction of descendent transaction does not affect the   $PR$ of transactions in $st_i''$ and  $PR(tx, st_{i+1}) > 0$. 
% The Equation~\ref{eqn:proof:2} holds, and we conclude the proof for Case 2.


% For case 3), it is to prove,
% \begin{equation}
% \label{eqn:proof:3}
% \sum_{tx'\in{}st_i''} PR(tx', st_{i+1})
% \nonumber
% \\ 
% \geq \sum_{tx'\in{}st_i''} PR(tx', st_i) 
% \end{equation} 

% Because admission or eviction of descendent transaction does not affect the $PR$ of transactions in $st_i''$ 
% The Equation~\ref{eqn:proof:3} holds, and we conclude the proof for Case 3.

% We prove that Equation~\ref{eqn:iterative:i} holds, and for any state $st_n$, by iteratively applying this inequality, we can prove that the sum of $PR$ monotonically increases. 
% % Formally,

% \end{proof}



\begin{theorem}[$g$-eviction security of Algorithm~\ref{alg:adTx:AA:framework}]
\label{thm:policya:eviction}
A mempool running Algorithms~\ref{alg:adTx:AA:framework} is $g$-eviction secure. That is, given a sequence of arriving normal and adversarial transactions $\vec{ops}$ to the mempool state, the total transaction fees in the end-state mempool under attacks $st_n$ are lower-bounded by the following:

\begin{eqnarray}
\forall st_0, \vec{ops}, fees(st_n) &\geq{}& g(st_0) 
\label{eqn:mf:bound}
\end{eqnarray}
\end{theorem}


\begin{proof}
Due to Lemma~\ref{thm:pr:mono}, we prove the property of increasing sum of transaction prices during the mempool state transition, that is, Equation~\ref{eqn:iterative:n}. 

And the minimal gas for each transaction is $21000$. We have a lower bound for transaction $fee$ which is $21000\cdot{}tx.price$, that is,

\begin{eqnarray}
\nonumber
& fees(\vec{st_n}) \geq{} 21000\cdot{}\sum_{tx\in{}st_n}tx.price & 
\\ 
\nonumber
& \geq{} 21000\cdot{}\sum_{tx\in{}st_n} tx.price & 
\\ 
\label{eqn:cp:bound}
& \geq{} 21000\cdot{}\sum_{tx\in{}st_0} tx.price & 
\end{eqnarray}

Equation~\ref{eqn:mf:bound} holds.
\end{proof}

\subsection{Locking Insecure of $PR$}

% Policy \textsc{saferAd}-$PR$ is not locking secure.
% Figure~\ref{fig:moex2} shows a counterexample in which we can easily construct an effective locking attack. Specifically, recall that in the figure, $tx_3$ is declined by the mempool running Policy \textsc{saferAd}-$PR$ (i.e., Algorithm~\ref{alg:adTx:AA:framework} with $score_{\textsc{saferAd}-$PR$}$). Assume transactions $tx_1$ and $tx_2$ are sent by an adversary (i.e., Adversarial account $A$), and $tx_3$ is sent by a benign user ($B$). This admission event implies that a benign user's transaction of price $4$ is declined by a mempool where the average transaction price per slot is $\frac{1+5}{2}=3$, which is lower than $4$. Suppose there is another subsequent normal transaction $tx_5=\langle{}D1, 4\rangle{}$. $tx_5$ would be declined by the mempool. Had $tx_3$ and $tx_5$ been admitted into the mempool, the sum of prices in the end state would have been $4+4=8$, which is higher than the sum of prices in the actual mempool end state, $1+5=6$. This is an asymmetric mempool-locking attack. 
% Note that the example here also violates $h$-locking security where $h$ must be lower than the average transaction price.


% A mempool running Algorithms~\ref{alg:saferadP} is locking insecure. 

Policy \textsc{saferAd}-$PR$ is not locking secure. We illustrate this with a counterexample that highlights how an attacker can exploit policy $PR$ to achieve a denial-of-service (DoS) with minimal cost.

Consider a mempool implementation that imposes no limitations on the number of transactions sent by a single sender. Suppose the mempool is at full capacity, and all transactions originate from a single sender. These transactions are represented as: $tx_1, tx_2, \ldots, tx_{n-1}$, each with a price of 1, while the only transaction without child dependencies, $tx_n$, has the highest nonce and a significantly higher price of 10,000.

The mempool operates under policy $PR$ where an incoming transaction $tx_a$ can only evict an existing transaction if $tx_a$ has a higher price than the transaction it aims to evict. Given this policy, $tx_a$ would need a price greater than 10,000 to evict $tx_n$. This creates a scenario where the attacker can effectively lock the mempool with a low-cost strategy by ensuring $tx_n$ remains in place, thus preventing the eviction of other transactions priced at 1.


% Here is a couter example. For a mempool without any limitation for the number of transactions sent by one sender, we suppose there is only one sender in the full mempool and its transactions are all have price 1 ($tx_1,...,tx_{n-1}$) except for the only childless transaction which is the transaction ($tx_n$) with the largest nonce has price 10000 that is way higher than the normal transaction price. Then, according to the eviction policy. The arriving transaction $tx_a$ could only evict $tx_n$ when its price higher than $tx_n$'s price 10000 which can cause the locking attack with the low cost of attacker. 

\section{Implementation Notes on Geth}

We build a prototype implementation of \textsc{saferAd}-$PR$ on Geth $v1.11.4$. We describe how the pending mempool in vanilla Geth handles transaction admission and then how we integrate \textsc{saferAd}-$PR$ into Geth.

\noindent{\bf
Background: Geth mempool implementation}: In Geth $v1.11.4$, the mempool adopts the price-only Policy patched with extra checks. Concretely, upon an arriving transaction $ta$, \circled{0} Geth first checks the validity of $ta$ (e.g., $ta$ is an overdraft), then it checks if the mempool is full. \circled{1} If so, it finds the transaction with the lowest price as the candidate of eviction victim $te'$. \circled{2} It then removes $te'$ from the primary storage and the secondary index. \circled{3} At last, it adds $ta$ to the primary storage and the secondary index.
If the mempool is not full, \circled{4} Geth adds $ta$ to the primary storage and to the secondary index.

For fast transaction lookup, Geth $v1.11.4$ maintains two indices to store mempool transactions (i.e., each transaction is stored twice): a primary index where transactions are ordered by price and a secondary index where transactions are ordered first by senders and then by nonces. 

In Step \circled{0}, we adopt the patch against MemPurge attacks~\cite{me:mempurge:fix}.

\noindent{\bf
Implementation of \textsc{saferAd}-$PR$ on Geth}: Geth's mempool architecture is well aligned with Algorithm~\ref{alg:adTx:AA:framework}.
We overwrite Step \circled{1} in Geth; instead of finding the transaction with the lowest price, we find the childless transaction with the lowest price, which is to scan Geth's price-based index from the bottom, that is, the transaction with the lowest price; for each transaction, we check if the transaction has a defendant in the mempool by querying the second index. If so, we continue to the transaction above in the primary index and repeat the check. If not, we select the transaction to be eviction victim $te$. Steps \circled{2}, \circled{3}, and \circled{4} remain the same except that reference $te'$ is replaced with $te$.


\section{Revenue Evaluation}

\subsection{Experimental Setups}
\label{sec:setup}

\noindent{\bf Workload collection}: 
For transaction collection, we first instrumented a Geth client (denoted by Geth-m) to log every message it receives from every neighbor. The logged messages contain transactions, transaction hashes (announcements), and blocks. When the client receives the same message from multiple neighbors, it logs it as multiple message-neighbor pairs. We also log the arrival time of a transaction or a block.


We ran a Geth-m node in the mainnet and collected transactions propagated to it from Sep. 5, 2023 to Oct. 5, 2023. In total, $1.5*20^8$ raw transactions are collected, consuming $30$ GB-storage. 
We make the collected transactions replayable as follows: We initialize the local state, that is, account balances and nonces by crawling relevant data from infura.io. We then replace the original sender in the collected transactions with the public keys that we generated. By this means, we know the secret keys of transaction senders and are able to send the otherwise same transactions for experiments. 

We choose $8$ traces of consecutive transactions from the raw dataset collected, each lasting $2.5$ hour. We run experiments on each $2.5$-hour trace. The reason to do so, instead of running experiments directly on the one-month transaction trace, is that the initialization of blockchain state in each trace requires issuing RPC queries (e.g., against infura) on relevant accounts, which is consuming; for a $2.5$-hour trace, the average time of RPC querying is about one day. To make the selected $2.5$-hour traces representative, we cover both weekdays and weekends, and on a single day, daytime and evening times.


\begin{figure}[!bthp]
\centering
%\includegraphics[width=0.375\textwidth]{figures/exp-setup.eps}
\includegraphics[width=0.375\textwidth]{figures/exp-setup2.eps}
\caption{Experimental setup}
\label{fig:exp:setup}
\end{figure}

\noindent{\bf Experimental setup}:
For experiments, we set up four nodes, an optional attack node sending crafted transactions, a workload node sending normal transactions collected, a victim non-validator node propagating the transactions and blocks between attack node and victim validator node, and a victim validator node receiving transactions from the workload node and attack node through non-validator node. The victim validator node is connected to both the workload node and victim non-validator node which is connected to the attack node. There is no direct connection between the attack node and the workload node. The attack node runs an instrumented Geth $v1.11.4$ client (denoted by Geth-a) that can propagate invalid transactions to its neighbors. The victim nodes runs the target Ethereum client to be tested; we tested two victim clients: vanilla Geth $v1.11.4$ and \textsc{saferAd}-$PR$ $PR$; the latter one is implemented as addon to Geth $v1.11.4$. The workload node runs a vanilla Geth $v1.11.4$ client. On each node, we also run a Prysm $v3.3.0$ client at the consensus layer. The experiment platform is depicted in Figure~\ref{fig:exp:setup}.
Among the four nodes, we stake Ether to the consensus-layer client on the victim validator node, so that only the victim validator node would propose or produce blocks. 

We run experiments in two settings: under attacks and without attacks. For the former, we aim at evaluating the security of \textsc{saferAd}-$PR$ under attacks, that is, how successful DoS attacks are on \textsc{saferAd}-$PR$. In this setting, we run all three nodes (the victim, attacker and workload nodes). For the latter, we aim at evaluating the utility of \textsc{saferAd}-$PR$ under normal transaction workloads. In this setting, we only run victim and workload nodes, without running the attack node.

In each experiment, 1) we replay the collected transactions as follows: For each original transaction $tx$ collected, we send a replayed transaction $tx'$ by replacing its sender with a self-generated blockchain address. $GasUsed$ is simulated: If $tx$ runs a smart contract, $tx'$ does not run the same contract. Instead, we make $tx'$ run our smart contract with $tx'.GasUsed$ equals $tx.GasUsed$ if $tx$ is included in the mainnet blockchain, or equal $tx.Gas$ (i.e., the Gas limit set by the transaction sender) if $tx$ is not included.
2) When replaying a collected block, we turn on the block-validation function in Prysm, let it produce and validate one block, and send the block (which should be different from the content of the collected block) to the Geth client. We then immediately turn off block validation before replaying the next transaction in the trace.


\subsection{Revenue Under Normal Transactions}

This experiment compares different mempool policies by evaluating their block revenue under the same transaction workloads. 

\noindent{\bf Experimental method}: We consider two mempool policies, the baseline one in Geth $v1.11.4$ and \textsc{saferAd}-\textsc{PR} on the baseline. Given each policy, we replay the $8$ transaction traces in the same way as before and collect the produced blocks. We report the average revenue per block collected from the blocks. 

\noindent{\bf Results}: Figure~\ref{fig:Revenue_block_real_trace} presents the revenue of the selected $150$ consecutive blocks from the $600$ blocks in Trace $2$. The numbers of the three mempool policies are close, and they fluctuate in a similar way. 
Table~\ref{tab:revenue:8traces} presents the aggregated results by the total revenue and revenue per block. Compared to Geth $v1.11.4$, Policy \textsc{PR}'s revenue per block falls in the range of $[100\%+1.18\%, 100\%+7.96\%]$. This result suggests \textsc{saferAd}-$PR$ incurs no significant change of block revenue under normal transactions.


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.38\textwidth]{figures/Revenue_block_real_trace_short.eps}
  \caption{Block revenue w/w.o. \textsc{saferAd}-$PR$ under Trace $1$.}
\label{fig:Revenue_block_real_trace}
\end{figure}

\begin{table}[!htbp]
\caption{Average block revenue (Ether) of different mempool policies. In bold are max and min numbers.}
\label{tab:revenue:8traces}
\centering{\scriptsize
\begin{tabularx}{0.4\textwidth}{|c|X|c| }
\hline 
% Tx   & \multicolumn{1}{l}{Policy \textsc{AP} (Ether)} & \multicolumn{1}{l}{Geth (Ether)}  \\ \cline{2-5}
Trace &  \textsc{PR} (Ether) 
% & \textsc{AP}  
% & $AP2$ 
& Geth (Ether)\\ \hline
1  
&$0.73\ (+3.13\%)$
% &$0.72\ (+1.02\%)$
% &$0.7\ (-0.73\%)$
&$0.71$	 \\ \hline
2
&$1.17\ (+6.97\%)$
% &$1.08\ (-1.19\%)$
% &$1.09\ (+0.27\%)$
&$1.09$	\\ \hline
3 
&$0.85\ (+4.55\%)$
% &$0.81\ (-0.21\%)$	
% &$0.8\ (-0.67\%)$
&$0.81$	 \\ \hline
4
&$0.54\ (+4.56\%)$
% &\textbf{0.54 (+2.55\%)}	
% &\textbf{0.53 (+1.96\%)}
&$0.52$	 \\ \hline   
5 
&$0.78\ (+6.66\%)$
% &$0.72\ (-1.09\%)$	
% &$0.74\ (+0.91\%)$
&$0.73$	 \\ \hline
6 
&$1.19\ (+4.23\%)$
% &\textbf{1.12 (-1.33\%)}
% &$1.13\ (-0.83\%)$
&$1.14$	 \\ \hline
7   
&\textbf{0.56 (+1.18\%)}
% &$0.57\ (+2.1\%)$	
% &\textbf{0.54 (-1.85\%)}
&$0.55$	 \\ \hline
8 
&\textbf{0.64 (+7.96\%)}
% &$0.59\ (+0.74\%)$	
% &$0.6\ (+0.96\%)$
&$0.59$	 \\ \hline
\end{tabularx}
}
\end{table}


% \begin{table}[!htbp]
% \caption{Block revenue of 8 real transaction traces under different policies. Bold are max and min numbers.}
% \label{tab:revenue:8traces}
% \centering{\small
% \begin{tabularx}{0.495\textwidth}{|c|C|X|c|c| }
% \hline 
% Tx   & \multicolumn{2}{l|}{Policy $PR$ (Ether)} & \multicolumn{2}{l|}{Geth (Ether)}  \\ \cline{2-5}
% trace & Total revenue & Revenue per block & Total &Per block \\ \hline
% 1 & 
% $429.38$	&$0.72 (+1.02\%)$
% &$425.04$	&$0.71$	 \\ \hline
% 2&
% $647.25$	&$1.08 (-1.19\%)$
% &$655.05$	&$1.09$	\\ \hline
% 3 &
% $487.55$	&$0.81 (-0.21\%)$	
% &$488.57$	&$0.81$	 \\ \hline
% 4 &
% $322.66$	&\textbf{0.54 (+2.55\%)}	
% &$314.63$	&$0.52$	 \\ \hline   
% 5 &
% $430.31$	&$0.72 (-1.09\%)$	
% &$435.05$	&$0.73$	 \\ \hline
% 6 &
% $674.48$	&\textbf{1.12 (-1.33\%)}	
% &$683.57$	&$1.14$	 \\ \hline
% 7  & 
% $339.68$	&$0.57 (+2.1\%)$	
% &$332.69$	&$0.55$	 \\ \hline
% 8 &
% $355.25$	&$0.59 (+0.74\%)$	
% &$352.64$	&$0.59$	 \\ \hline
% \end{tabularx}
% }
% \end{table}


\subsection{Revenue Under Attacks}
\label{sec:setup:singlenode}

\noindent{\bf Background of attacks}: This experiment evaluates the security of \textsc{saferAd}-$PR$ against known attacks. Given that our implementation is on Geth $v1.11.4$, we choose the attacks still effective on this version: $XT_6$~\cite{wang2023understanding}. Briefly, the attack works in four steps: 1) It first evicts the Geth mempool by sending $384$ transaction sequences, each of $16$ transactions from a distinct sender. The transaction fees are high enough to evict normal transactions initially in the mempool. 2) It then sends $69$ transactions to evict $69$ parent transactions sent in step 1) and turn their child transactions into future transactions. 3) Since now there are more than $5120$ pending transactions in the mempool, Geth's limit of $16$ transactions per send is off. It then conducts another eviction; this time, it sends all $5120$ transactions from one sender, evicting the ones sent in the previous round. 4) At last, it sends a single transaction to turn all transactions in the mempool but one into future transactions. The overall attack cost is low, costing the fee of one transaction.

Because $XT_6$ can evict Geth's mempool to be left with one transaction, we use as Geth's bound the maximal price in a given mempool times the maximal Gas per transaction (i.e., block Gas limit, namely $30$ million Gas).

\noindent{\bf Experimental method}: We set up the experiment platform described in \S~\ref{sec:setup:singlenode}. In each experiment, we drive benign transactions from the workload node. Note that the collected workload contains the timings of both benign transactions and produced blocks. On the $30$-th block, we start the attack. The attack node observes the arrival of a produced block and waits for $d$ seconds before sending a round of crafted transactions. 

The attack phase lasts for $36$ blocks; after the $66$-th block, we stop the attack node from sending crafted transactions. We keep running workload and victim nodes for another $24$ blocks and stop the entire process at the $90$-th block. We collect the blocks produced and, given a block, we report the total fee of transactions included. 

\begin{figure}[!ht]
  \centering
  \subfloat[$XT_6$ w. $8$-sec. delay (single node)]{%
\includegraphics[width=0.225\textwidth]{figures/saferad-attack-evaluation1.eps}
    \label{fig:saferad-attack-eval}
    \label{fig:successrate-geth}}%
  \subfloat[$XT_6$ w. varying delay (single node)] {%
   \includegraphics[width=0.225\textwidth]{figures/saferad-attack-varying-delay1.eps}
  \label{fig:delay-geth}}
  \caption{Validator revenue under attacks: With and without \textsc{saferAd}-$PR$ defenses.}%
\end{figure}

\noindent{\bf Results}: Figure~\ref{fig:saferad-attack-eval} reports the metrics for $XT_6$ on two victim clients: vanilla Geth $v1.11.4$ and \textsc{saferAd}-$PR$. Before the attack is launched (i.e., before the $30$-th block), the two clients produce a similar amount of fees for benign transactions, that is, around $0.7 - 2.0$ Ether per block. As soon as the attack starts from the $30$-th block, Geth's transaction fees quickly drop to zero Ether, which shows the success of $XT_6$ on unpatched Geth $v1.11.4$. There are some sporadic spikes (under $0.7$ Ether per block), which is due to that $XT_6$ cannot lock the mempool on Geth. 
Patching Geth with \textsc{saferAd}-$PR$ can fix the vulnerability. After the attack starts on the $30$-th block, the transaction fees, instead of decreasing, actually increase to a large value; the high fees are from adversarial transactions and are charged to the attacker's accounts. The high fees show the effectiveness of \textsc{saferAd}-$PR$ against known eviction-based attacks ($XT_6$).



Figure~\ref{fig:delay-geth} shows the total fee per block under $XT_6$ with varying delays, where the delay measures the time between when a block is produced and when the next attack arrives.
The results of Geth $v1.11.4$ show that with a short delay, the total transaction fees in mempool are high because $XT_6$ cannot lock a mempool, and the short block-to-attack delay leaves enough time to refill the mempool. With a median delay (e.g., sending an attack $8$ seconds after a block is produced), the attack is most successful, leaving mempool at zero Ether. With a long delay, the in-mempool transaction fees grow high due to the attack itself being interrupted by the block production. Under varying delays, the transaction fees of the mempool practicing \textsc{saferAd}-$PR$ policy would remain constant at a high value, showing the defense effectiveness against attacks of varying delays.


\subsection{Estimation of Eviction Bounds}
\label{sec:eval:eviction:bounds}

% {\color{blue}

% }

% This experiment evaluates the eviction bound of \textsc{saferAd}-$PR$, as in Equation~\ref{eqn:mf:bound}, under real-world transaction workloads. 

% Our goal is to understand whether bounding mempool fees using Equation~\ref{eqn:mf:bound} ensures the failure of known ADAMS attacks. In that regard, we also include a baseline, namely, the fees of an unprotected mempool under a successful ADAMS attack.

% \ignore{
% This experiment quantitatively evaluates the different eviction fee bounds for \textsc{saferAd}-$PR$ and unprotected Geth $v1.11.4$. Recall that the lower bound of transaction fees for \textsc{saferAd}-$PR$ is dependent on the benign transaction workloads (e.g., $st_{nb}$ as in Equation~\ref{eqn:mf:bound}). We evaluate the bound in the equation on real-world transaction traces collected from the mainnet.
% }

% % comparing with the total fees in the mempool without attack
% % For vanilla Geth $v1.11.4$, as mentioned in Section $5.3$, the mempool fees under $XT_6$ attack correspond to the fee of the highest-priced transaction that remains.



% In this experiment, we replayed eight real-world transaction traces to test two Ethereum clients: vanilla Geth $v1.11.4$ and Geth hardened with \textsc{saferAd}-$PR$. We replayed the traces on vanilla Geth $v1.11.4$ twice and on \textsc{saferAd}-$PR$ once. On each run, we captured snapshots every 30 seconds and evaluated the following metrics: 
% 1) \textsc{saferAd}-$PR$ fee bound: the eviction bound estimate using Equation~\ref{eqn:mf:bound}. 
% 2) Geth fees without attacks: that is  the total deterministic transaction fees in vanilla Geth $v1.11.4$ client without any attack. 
% 3) Geth fees with $XT_6$ attacks: that is the transaction fees in Geth $v1.11.4$ under $XT_6$ attack, where the mempool is evicted to a single transaction with the highest price.

% In the experiment, we test given clients: a vanilla Geth $v1.11.4$ and Geth hardened by \textsc{saferAd}-$PR$. Given a tested client, we replay the collected eight transaction traces described in \S~\ref{sec:setup}. We take a snapshot every $30$ seconds, and estimate the lower bounds using the derived equation (Equation~\ref{eqn:mf:bound}). At each time point, given a mempool state $st$, we record three metrics: Total mempool fees in vanilla Geth $v1.11.4$ without attack, the eviction bound estimated from the \textsc{saferAd} mempool, and the mempool fees of vanilla Geth $v1.11.4$ under the $XT_6$ attack (the baseline). For the baseline, since $XT_6$ can evict the mempool to a single transaction, we conservatively use the transaction of the highest price in a mempool to estimate the fees.

This experiment estimates the eviction bounds of different admission policies under real-world transaction workloads. 

\noindent{\bf Experimental method}: In the experiment, we replayed the transaction traces we collected in \S~\ref{sec:setup} each of two Ethereum clients, be it either $PR$, or vanilla Geth $v1.11.4$ . In each run, right after producing each block, say $bk_i$, we record the mempool snapshot $st_i$. Then, assuming an attack starts right after the block $bk_i$ is produced and lasts for the next $10$ blocks, we estimate the lower bound of fees in the mempool right after block $bk_{i+10}$ under arbitrary eviction attacks.

1) For $PR$, we use Equation~\ref{eqn:cp:bound} as the estimation bound.
2) For the baseline, we consider vanilla Geth $v1.11.4$ under $XT_6$; instead of mounting actual attacks (which is time-consuming), we estimate the attack damage by considering that the mempool under attack contains only one transaction, which is consistent with the mempool end-state under an actual $XT_6$ attack.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.38\textwidth]{figures/Block_revenue_lower_bound_short.eps}
  \caption{Block revenue lower bounds.}
\label{fig:Block_revenue_lower_bound_short}
\end{figure}

\begin{table}[!htbp]
\caption{Average, $95$-th, and $5$-th percentile of eviction bounds under different policies on eight transaction traces}
\label{tab:eviction:bound}
\centering{\small
\begin{tabularx}{0.4\textwidth}{|l|X|X|X|}
\hline 
  & Avg. bound (Ether) & $95\%$ bound (Ether) & $5\%$ bound (Ether) \\ \hline
$PR$ & $6.05$	&$13.72$	&$2.63$ \\ \hline
% \textsc{AP} & $101.05$	&$299.60$	&$16.41$ \\ \hline
% $AP2$ & $87.46\%$	&$92.32\%$	&$80.37\%$ \\ \hline
Geth & $0.63\cdot{}10^{-3}$	&$1.05\cdot{}10^{-3}$	&$0.17\cdot{}10^{-3}$ \\ \hline
\end{tabularx}
}
\end{table}


\noindent{\bf 
Results}: 
Figure~\ref{fig:Block_revenue_lower_bound_short} presents the results of estimated bounds over time. Compared to the mempool fees post attacks in Geth $v1.11.4$, both \textsc{saferAd} policies achieve high eviction bounds. The bound of $PR$ is higher than that of Geth $v1.11.4$ by $4$ orders of magnitude.
Table~\ref{tab:eviction:bound} presents statistics of the estimated bounds on the two clients tested. It includes the average, $95$-th, and $5$-th percentile of eviction bounds. \textsc{saferAd}-$PR$ achieves statistically higher bounds than the baseline of Geth. On average, $PR$'s eviction bound is $6.05$ Ether, which is much higher than the $0.63\cdot{}10^{-3}$ Ether in Geth under attacks.
And specifically, for $PR$, 5\% of its bounds exceed $13.72$ Ether, and 95\% exceed $2.63$ Ether.

% Figure~\ref{fig:Block_revenue_lower_bound_ndss} reports the timeline results of trace 2 across different clients. The figure illustrates that \textsc{saferAd}-$PR$ tightly bounds the Geth fees without attack, with \textsc{saferAd}-$PR$'s bounds being significantly higher compared to the original vanilla Geth client with $XT_6$ attack (baseline), by up to 4 orders of magnitude.

% Table~\ref{tab:eviction:bound} presents the average and percentile of the ratio $Rt$ on each mempool snapshots $st$ across eight traces. The ratio is calculated as follows,
% \begin{eqnarray}
%     Rt(st) = \frac{g(st)}{21000\cdot{}\sum_{tx\in{}st}tx.price}
% \end{eqnarray}

% Our observations indicate that the bound provided by \textsc{saferAd}-$PR$ is high as deterministic fee. Across 8 traces, $PR$ has ratio of 100\%.


% Table~\ref{tab:eviction:bound} presents the percentage of ratio for estimated fee bound under eviction attacks to mempool fees without attack across eight traces.
% Based on our observations, the bounds provided by \textsc{saferAd} are notably high. Specifically, we found that only 5\% of the snapshots have a lower bound that is less than 7.3\% of mempool fees without attack. Additionally, the average bound reaches $34.18\%$  of mempool fees, and remarkably, $5\%$ of lower bounds are higher than $71\%$ of mempool fees.

% \begin{table}[!htbp]
% \caption{Average and percentile of ratios of fee bound (with attack) to deterministic $Geth$ fees (w.o. attack) under different policies across eight transaction traces}
% \label{tab:eviction:bound}
% \centering{\small
% \begin{tabularx}{0.4\textwidth}{|l|X|X|X|}
% \hline 
% & Avg. & $95\%$ & $5\%$\\ \hline
% \textsc{saferAd}-$PR$ & $100\%$	&$100\%$	&$100\%$ \\ \hline
% Geth & $2.2\cdot{}10^{-5}$	& $4.2\cdot{}10^{-5}$ &$8\cdot{}10^{-6}$ \\ \hline
% \end{tabularx}
% }
% \end{table}


\section{Performance Evaluation}
\subsection{Platform Setup}

In this work, we use Ethereum Foundation's test framework~\cite{me:txpooltest} to evaluate the performance of the implemented countermeasures on Ethereum clients. Briefly, the framework runs two phases: In the initialization phase, it sets up a tested Ethereum client and populates its mempool with certain transactions. In the workload phase, it runs multiple ``rounds'', each of which drives a number of transactions generated under a target workload to the client and collects a number of performance metrics (e.g., latency, memory utilization, etc.). In the end, it reports the average performance by the number of rounds.
In terms of workloads, we use one provided workload (i.e., ``Batch insert'') and implement our own workload (``Mitigated attacks'').


\subsection{Experimental Results}

\noindent{\bf Workload ``Batch insert''}: 
We use the provided workload "Batch insert" that issues \texttt{addRemote} calls to the tested \texttt{txpool} of the Geth client. We select this workload because all our countermeasures are implemented inside the \texttt{addRemote} function. In the initialization phase, this workload sends no transaction to the empty mempool. In the workload phase, it runs one round and sends $n_0$ transactions from one sender account, with nonces ranging from $1$ to $n_0$, and of fixed Gas price $10000$ wei. When $n_0$ is larger than the mempool size, Geth admits the extra transactions to the mempool, buffers them, and eventually deletes them by running an asynchronous process that reorg the mempool (i.e., Function \texttt{pool.scheduleReorgLoop()} in Geth).

\begin{figure}[!ht]
\centering
\subfloat[Workload ``Batch insert'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_BatchInsert_short.eps}
   % \includegraphics[width=0.45\textwidth]{figures/wanning.eps}
    \label{fig:mentor-case}}
\subfloat[Workload ``Mitigated attack TN1'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_TD1_short.eps}
    \label{fig:corner-td1}}%
\caption{Running time of \textsc{saferAd}-$PR$ on Geth $v1.11.4$}%
\end{figure}

\begin{figure}[!ht]
\centering
\subfloat[Workload ``Batch insert'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_BatchInsert_memory_short.eps}
   % \includegraphics[width=0.45\textwidth]{figures/wanning.eps}
    \label{fig:mentor-case_memory}}
\subfloat[Workload ``Mitigated attack TN1'']{%
    \includegraphics[width=0.25\textwidth]{figures/bench_TD1_memory_short.eps}
    \label{fig:corner-td1_memory}}%
\caption{Memory usage of \textsc{saferAd}-$PR$ on Geth $v1.11.4$}%
\end{figure}

{
%\color{red}
We report running time and memory usage in Figure~\ref{fig:mentor-case} and Figure~\ref{fig:mentor-case_memory}, respectively. In each figure, we vary the number of transactions $n_0$ from $1000$ to $10000$, where $n_0 \in [1000, 5000]$ indicates a non-full mempool, and $n_0 \in [5000, 10000]$ indicates a full mempool. It is clear that on both figures, the performance overhead for a non-full mempool is much lower than that for a full mempool; and when the mempool is full, both the running time and memory usage linearly increase with $n_0$. The high overhead is due to the expensive mempool-reorg process triggered by a full mempool.
Specifically, 1) upon a full mempool ($n_0>5000$), on average, Geth $v1.11.4$ hardened by \textsc{saferAd}-$PR$ causes $1.073\times$ running time and $1.000\times$ memory usage, compared to vanilla Geth $V1.11.4$.
2) When the mempool is not full ($n_0\leq{}5000$), on average, Geth $v1.11.4$ hardened by \textsc{saferAd}-$PR$ causes $1.017\times$ running time and $1.000\times$ memory usage, compared to vanilla Geth $V1.11.4$.
Overall, the performance overhead introduced by \textsc{saferAd}-$PR$ is negligible.
} 

Note that Geth $v1.11.4$ that mitigates DETER causes $1.083\times$ running time compared to vanilla Geth $v1.11.3$, which is vulnerable to DETER. 


\noindent{\bf Workload ``Mitigated attack TN1''}: 
We additionally extend the framework with our custom workloads for countermeasure evaluation. Here, we describe the performance under one custom workload, "Mitigated attack TN1".

In the initialization phase, it first sends $n_1$ pending transactions to an empty mempool sent from $n_1'$ accounts, each of which has transactions of nonces ranging from $1$ to $\frac{n_1}{n_1'}$. All the parent transactions of nonce $1$ are of Gas price $1,000$ wei, and the others are of $200,000$ wei. It then sends $1024$ future transactions and $5120-n_1$ pending transactions from different accounts, all with nonce $1$, to fill the mempool. In the workload phase, it sends $n_1'$ transactions, each of price $20,000$ wei, to evict the parents and turn children into future transactions. 

In each experiment, we fix $n_1'$ at $10$ accounts and vary $n_1$ to be $10, 100, 1000$ and $4000$. We run the workload ten times and report the average running time and memory used with the standard deviation, as in Figure~\ref{fig:corner-td1} and Figure~\ref{fig:corner-td1_memory}. The running time and memory used are insensitive to the number of transactions ($n_1$). The performance overhead introduced by \textsc{saferAd}-$PR$ is negligible.

==> text/wanning-proof.tex <==

\newpage
\section{Proof of Mempool Order-Insensitivity}

\begin{lemma} \label{lemma:1}
Consider a mempool of Algorithms~\ref{alg:saferad} and~\ref{alg:saferadA} runs any timeline $st_1=f(\langle{}st_0\rangle{}, tx_a)$, $st_2=f(\langle{}st_1\rangle{}, tx_b)$, and its transaction-``reordered'' timeline $st_1'=f(\langle{}st_0\rangle{}, tx_b)$, $st_2'=f(\langle{}st_1'\rangle{}, tx_a)$. If $mdf(st_1)=mdf(st_0)=mdf(st_1')$, 
$st_2\equiv{}st_2'$.
\end{lemma}


{\color{blue}
\ignore{
\section{The Mempool Order-Agnostic Theorem Definition and Proof}
\begin{theorem}[The Mempool Order-Agnostic Theorem]
\label{thm:The_Mempool_Order_Agnostic}
As illustrated in Figure~\ref{fig:mempool_state_transition}, given the initial mempool state $st_0$, incoming transactions $tx_a$ and $tx_b$ are sent from different senders sequentially, where $tx_a$ precedes $tx_b$, the intermediate state transitions to $st_1$ and eventually to $st_2$. Conversely, if $tx_b$ is sent before $tx_a$, the intermediate state becomes $st_1'$, leading to $st_2'$. Despite these different intermediate states, the final mempool states $st_2$ and $st_2'$ are identical.

\end{theorem}
}



% \begin{lemma}[Final State Invariance]
    % \label{lem:Final_State_Invariance}
    % A mempool is final state invariance means that it will reach identical final states ($st_2$, $st_2'$) regardless of the order of arriving $txs$(i.e., $tx_a,tx_b$ or $tx_b,tx_a$), if the minimum fee of intermediate states ($st_1$, $st_1'$) right after the arrival of the first $tx$($tx_a$ or $tx_b$), remains unchanged from the initial state $st_0$. That is: $\forall{}st_0, st_1, st_1', st_2, st_2'$
    % \begin{eqnarray}
    % \min_{\forall{}tx\in{}st_0} tx.fee = 
    % \min_{\forall{}tx\in{}st_1} tx.fee = \min_{\forall{}tx\in{}st_1'} tx.fee\\
    % => st_2 = st_2'
    % \end{eqnarray}
    % \end{lemma}

    \begin{proof}
    We have 
    \begin{eqnarray}
    mdf(st_1)=mdf(st_0)=mdf(st_1')
    \end{eqnarray} 
    
    Then for $tx_a$ and $tx_b$ in two timelines, the condition of ckEvict/ckAdmit is 
    \begin{eqnarray}
    tx_a.fee>mdf(st_0), \\
    tx_a.fee>mdf(st_1') = mdf(st_0),\\
    tx_b.fee>mdf(st_1) = mdf(st_0), \\
    tx_b.fee>mdf(st_0)
    \end{eqnarray}
    For a given transaction $tx_a$, the decisions across both timelines are the same (i.e., both admitted or evicted) because the conditions are identical. This principle also applies to $tx_b$.

    Additionally, the evicted transactions are consistent. If one or two transactions are to be evicted while admitting $tx$, they must be the last or last and second-to-last child transactions in the same account transaction list as $mtx$ with the minimum fee.
    
    Therefore, for the two timelines, the admitted transactions are consistent, as are the evicted transactions, resulting in the same final states. In other words, $st_2\equiv{}st_2'$.
    \end{proof}



    \begin{lemma}[mf-Partially Filled Minimum Fee Preservation]
    \label{lem:mf:Minimum_Fee_Preservation}
    For any pair of transactions $tx_a$ and $tx_b$ arriving at a partially filled mempool($st_0$) under policy mf, $st_1$, $st_1'$ represent the intermediate state after admitting either $tx_a$ or $tx_b$. Then, it holds that:
    \begin{eqnarray}
        mdf(st_1)=mdf(st_0)=mdf(st_1')
        \label{eqn:mf:minimum_fee_perserve}
    \end{eqnarray} 
    \end{lemma}

    \begin{proof}
       If the first arriving $tx_a$ is declined, the state remains unchanged: $st_1 = st_0$, if $tx_a$ is admitted, it doesn't evict any $tx$ in the mempool because there is at least one empty slot, and $tx_a.fee > mdf(st_0)$, so that, 
       \begin{eqnarray}
       mdf(st_1)=mdf(st_0)
       \end{eqnarray} 
        Correspondingly, the arriving $tx_b$ have the same property, so that,
        \begin{eqnarray}
        mdf(st_0)=mdf(st_1')
        \end{eqnarray}
        As a result, Equation~\ref{eqn:mf:minimum_fee_perserve} holds.
    \end{proof}



    \begin{lemma}[mf-Full-Non-child Minimum Fee Preservation]
    \label{lem:mf:Minimum_Fee_Preservation_full}
    Given a full mempool under policy mf where the $mtx$ with minimum fee in initial state $st_0$ is not a child $tx$, if two $txs$($tx_a$, $tx_b$) arrives at the mempool in different orders, then the minimum fee of the intermediate state($st_1$ or $st_1'$) after admitting either $tx_a$ or $tx_b$ remains unchanged from the initial state. That is:
    \begin{eqnarray}
        mdf(st_1)=mdf(st_0)=mdf(st_1')
    \end{eqnarray} 
    \end{lemma}

    \begin{proof}
    The first arriving $tx$($tx_a$ or $tx_b$) is either admitted or declined.
    
    If it is declined, the intermediate state is same as initial state($st_1=st_0$ or $st_1'=st_0$), keeping the minimum fee unchanged.
    If it is admitted by evicting child $tx_e$(not $mtx$ itself) of $mtx$ with minimum fee, the $mtx$ with minimum fee doesn't change, as the minimum fee of intermediate state is still unaffected.
    Proof done.
    \end{proof}

    
\begin{proof}
    Here we prove the theorem demonstrating the Mempool's state insensitivity to the order of incoming transactions under Policy $mf$. 
    
    Regarding the initial state, two cases are considered: 1) the initial mempool is partially filled, and 2) the initial mempool is full.
    \begin{enumerate}
    \item For partially filled mempool, recall Lemma~\ref{lem:mf:Minimum_Fee_Preservation}, the intermediate state's minimum fee keeps same as initial state.
    Then recall Lemma~\ref{lem:Final_State_Invariance}, the final states $st_2 = st_2'$. 
    
    \item For full mempool, we consider two cases in this situation: a) the $mtx$ with minimal fee is not a child $tx$, b) the $mtx$ with minimal fee is child $tx$.
    \begin{enumerate}
        \item For full mempool and the $mtx$ with minimal fee is not a child (Lemma~\ref{lem:mf:Minimum_Fee_Preservation_full}), we also have unchanged minimum fee of intermediate states.
        Then recall Lemma~\ref{lem:Final_State_Invariance}, the final states keep same.

        \item we consider four cases for the decisions with arriving sequence $tx_a$, $tx_b$, i) both are declined, ii) both are admitted, iii) $tx_a$ is admitted while $tx_b$ is declined, iv) $tx_a$ is declined while $tx_b$ is admitted.
        \begin{enumerate}
            \item 
            We assume that $tx_a$ is declined first, so $tx_a.fee < mdf(st_0)$, leading to intermediate state:
            \begin{eqnarray} 
            st_1 \equiv{} st_0
            \end{eqnarray} 
            and $tx_b$ is also declined,  so $(tx_b.fee < mdf(st_1) = mdf(st_0))$, leading to end state:
            \begin{eqnarray} 
            st_2 \equiv{} st_1 \equiv{} st_0
            \end{eqnarray}


            Conversely, for sequence $tx_b$, $tx_a$, $tx_b$ is declined($tx_b.fee < mdf(st_0)$), leading to intermediate state:
            \begin{eqnarray} 
            st_1' \equiv{} st_0
            \end{eqnarray} 
            and $tx_a$ is also declined,  ($tx_a.fee < mdf(st_0) = mdf(st_1')$), leading to end state:
            \begin{eqnarray} 
            st_2' \equiv{} st_1' \equiv{} st_0
            \end{eqnarray}

            So $st_2 \equiv{} st_2'$.
                
            \item 
            We assume that $tx_a$ is admitted first and $mtx$ is child, $mtx$ is evicted and $tx_a.fee > mdf(st_0)$, leading to intermediate state:
            \begin{eqnarray} 
            st_1 \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\}
            \end{eqnarray} 
            Assuming $tx_b$ is also admitted, we discuss two cases: A) if the newly added $tx_a$ becomes the new $mtx(st_1)$, or
            B) the second minimum-fee transaction in the initial state, $mtx_2(st_0)$, becomes the new $mtx(st_1)$. 
            \begin{enumerate}
                \item  For $mtx(st_1) = tx_a$, $tx_a$ is evicted and $(tx_b.fee > tx_a.fee) \land (tx_a.fee < mtx_2(st_0))$ leading to the end state: 
                \begin{eqnarray}
                st_2 \equiv{} st_1 \cup \{tx_b\} \setminus \{tx_a\} \\
                \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
                \end{eqnarray} 
                
                Conversely, for sequence $tx_b$, $tx_a$, $tx_b$ is admitted by evicting $mtx(st_0)$ ($tx_b.fee > tx_a.fee > mdf(st_0)$) leading to the intermediate state:
                \begin{eqnarray}
                    st_1' \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
                \end{eqnarray}
                
                and $tx_a$ is declined($tx_a.fee < mtx_2(st_0)$) leading to the end state:
                \begin{eqnarray}
                   st_2' \equiv{} st_1' \\
                   \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\} 
                \end{eqnarray}
                So $st_2 \equiv{} st_2'$.

                
                \item For $mtx(st_1) = mtx_2(st_0)$, $mtx_2(st_0).child$ is evicted and $(tx_b.fee > mtx_2(st_0)) \land (tx_a.fee > mtx_2(st_0))$ leading to the end state: 
                \begin{eqnarray}
                st_2 \equiv{} st_1 \cup \{tx_b\} \setminus \{mtx_2(st_0).child\} \\
                \equiv{} st_0 \cup \{tx_a, tx_b\} 
                \setminus \{mtx(st_0), mtx_2(st_0).child\}
                \end{eqnarray} 
                
                Conversely, for sequence $tx_b$, $tx_a$, $tx_b$ is admitted by evicting $mtx(st_0)$ ($tx_b.fee > mtx_2(st_0) > mdf(st_0)$) leading to the intermediate state:
                \begin{eqnarray}
                    st_1' \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
                \end{eqnarray}
                
                and $tx_a$ is admitted by evicting $mtx_2(st_0).child$ ($tx_a.fee > mtx_2(st_0)$) leading to the end state:
                \begin{eqnarray}
                   st_2' \equiv{} st_1' \cup \{tx_a\} \setminus \{mtx_2(st_0).child\} \\
                   \equiv{} st_0 \cup \{tx_a, tx_b\} 
                   \setminus \{mtx(st_0), mtx_2(st_0).child\}
                \end{eqnarray}
                So $st_2 \equiv{} st_2'$.
            \end{enumerate}
           

            \item Same as case ii), we have intermediate state:
            \begin{eqnarray} 
            st_1 \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\}
            \end{eqnarray} 
            Assuming $tx_b$ is declined then, 
            we have end state:
            \begin{eqnarray} 
            st_2 \equiv{} st_1 \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\}
            \end{eqnarray} 

            Conversely, if $tx_b$ is declined first, we have intermediate state:
            \begin{eqnarray} 
            st_1' \equiv{} st_0
            \end{eqnarray} 
            Then $tx_a$ is admitted by evicting $mtx$($tx_a.fee > mdf(st_0) = mdf(st_1')$), we have end state:
            \begin{eqnarray} 
            st_2' \equiv{} st_1' \cup \{tx_a\} \setminus \{mtx(st_0)\} \\
            \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\}
            \end{eqnarray} 
            So $st_2 \equiv{} st_2'$.
            
            
            If the first $tx_b$ is admitted by evicting $mtx$, so the intermediate state:
                \begin{eqnarray}
                    st_1' \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
                \end{eqnarray}
            we discuss same two cases A), B) as case ii).
            \begin{enumerate}
                \item  For $mtx(st_1) = tx_a$, we have $(tx_b.fee < tx_a.fee) \land (tx_a.fee < mtx_2(st_0))\land (tx_b.fee > mdf(st_0))$.
                So $tx_a$ is admitted($tx_a.fee > tx_b.fee = mtx(st_1')$) by evicting $tx_b$ ($tx_b.fee < tx_a.fee < mtx_2(st_0)$) leading to the end state:
                \begin{eqnarray}
                   st_2' \equiv{} st_1' \cup \{tx_a\} \setminus \{tx_b\} \\
                   \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\} 
                \end{eqnarray}
                So $st_2 \equiv{} st_2'$.

                
                \item For $mtx(st_1) = mtx_2(st_0)$, we have $(tx_b.fee < mtx_2(st_0)) \land (tx_a.fee > mtx_2(st_0)) \land (tx_b.fee > mdf(st_0))$.
                 So $tx_a$ is admitted($tx_a.fee > mtx_2(st_0) > tx_b.fee = mtx(st_1')$) by evicting $tx_b$($tx_b.fee < mtx_2(st_0)$) leading to the end state:
                \begin{eqnarray}
                   st_2' \equiv{} st_1' \cup \{tx_a\} \setminus \{tx_b\} \\
                   \equiv{} st_0 \cup \{tx_a\} \setminus \{mtx(st_0)\} 
                \end{eqnarray}
                So $st_2 \equiv{} st_2'$.
            \end{enumerate}
            
            \item 
            Same as case i), we have intermediate state:
            \begin{eqnarray} 
            st_1 \equiv{} st_0 
            \end{eqnarray} 
            and $tx_b$ is admitted by evicting $mtx$, so $(tx_b.fee > mdf(st_1) = mdf(st_0))$, leading to end state:
            \begin{eqnarray} 
            st_2 \equiv{} st_1 \cup \{tx_b\} \setminus \{mtx(st_0)\}\\
            \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
            \end{eqnarray}


            Conversely, for sequence $tx_b$, $tx_a$, $tx_b$ is admitted by evicting $mtx$($tx_b.fee > mdf(st_0)$), leading to intermediate state:
            \begin{eqnarray} 
            st_1' \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
            \end{eqnarray} 
            and $tx_a$ is declined($tx_a.fee < mdf(st_0) < mdf(st_1') $), leading to end state:
            \begin{eqnarray} 
            st_2' \equiv{} st_1' \equiv{} st_0 \cup \{tx_b\} \setminus \{mtx(st_0)\}
            \end{eqnarray}

            So $st_2 \equiv{} st_2'$.
        \end{enumerate}
        
    \end{enumerate}
    \end{enumerate}

\end{proof}


}

==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table*}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

Table with diagbox

\begin{tabular}{|c|c|}
    \hline
    alghreaiog & bghsah \\
    \hline
    cagja & \notableentry \\
    \hline
    \cellcolor{blue} & edkhaklgjaj \\
    \hline
\end{tabular}

\begin{tabular}{|p{4cm}|p{3cm}|}
    \hline
    alghreaiog & bghsah \\
    \hline
    cagja\par bla & \notableentry \\
    \hline
    \cellcolor{blue} & edkhaklgjaj \par xyz \\
    \hline
\end{tabular}

Table line/cell/column colored

\begin{table}[ht]
\centering
\begin{tabular}{c|ccccccc}
\hline
& col1 & col2 & col3 & col4 & col5 & col6 & col7 \\
\hline
\rowcolor{LightCyan}
row1& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row2& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\rowcolor{LightCyan}
row3& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row4& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\rowcolor{LightCyan}
row5& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row6& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\hline
\end{tabular}
\end{table}

\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table}[ht]
\centering
\begin{tabular}{c|g|c|g|c|g|c|g}
\hline
&col1 &col2 &col3 &col4 & col5 &col6 &col7\\
\hline
row1& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row2& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row3& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row4& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row5& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row6& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\hline
\end{tabular}
\end{table}



\subsection{figures}
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5.eps}
\caption{Wrapped figure}
\label{fig:perf}
\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2.eps}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10.eps}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
    ...
    *Bitmap bm = BitmapFactory.decodeFile(file)*;
    return bm;
}

void EditPicture(Bitmap bm) {
    //heavy computational picture editing
    int i = 10 (* $*$ *); //escape to plot * literatelly instead of bolden text
    bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
    for(every pixel) {
      ...
    }  
    
    //embed location information into picture
    (* $*$*)Location loc = getLastKnownLocation(Provider)*;
    (* $*$*)double longitude = loc.getLongitude()*;
    (* $*$*)double latitude = loc.getLatitude()*;
    (* $*$*)EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}
\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}
\end{center}



\subsection{misc}
\begin{itemize}
  \item cmark $\cmark$ and xmark $\xmark$
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

